Risk-Aware Scene Sampling for Dynamic Assurance of Autonomous Systems

Autonomous Cyber-Physical Systems must often operate under uncertainties like sensor degradation and shifts in the operating conditions, which increases its operational risk. Dynamic Assurance of these systems requires designing runtime safety components like Out-of-Distribution detectors and risk estimators, which require labeled data from different operating modes of the system that belong to scenes with adverse operating conditions, sensors, and actuator faults. Collecting real-world data of these scenes can be expensive and sometimes not feasible. So, scenario description languages with samplers like random and grid search are available to generate synthetic data from simulators, replicating these real-world scenes. However, we point out three limitations in using these conventional samplers. First, they are passive samplers, which do not use the feedback of previous results in the sampling process. Second, the variables to be sampled may have constraints that are often not included. Third, they do not balance the tradeoff between exploration and exploitation, which we hypothesize is necessary for better search space coverage. We present a scene generation approach with two samplers called Random Neighborhood Search (RNS) and Guided Bayesian Optimization (GBO), which extend the conventional random search and Bayesian Optimization search to include the limitations. Also, to facilitate the samplers, we use a risk-based metric that evaluates how risky the scene was for the system. We demonstrate our approach using an Autonomous Vehicle example in CARLA simulation. To evaluate our samplers, we compared them against the baselines of random search, grid search, and Halton sequence search. Our samplers of RNS and GBO sampled a higher percentage of high-risk scenes of 83% and 92%, compared to 56%, 66% and 71% of the grid, random and Halton samplers, respectively.

==> Accepted/abstract.tex <==
\begin{abstract}
Autonomous Cyber-Physical Systems must often operate under uncertainties like sensor degradation and distribution shifts in the operating environment, thus increasing operational risk. Dynamic Assurance of these systems requires augmenting runtime safety components like out-of-distribution detectors and risk estimators. Designing these safety components requires labeled data from failure conditions and risky corner cases that fail the system. However, collecting real-world data of these high-risk scenes can be expensive and sometimes not possible. To address this, there are several scenario description languages with sampling capability for generating synthetic data from simulators to replicate the scenes that are not possible in the real world. Most often, simple search-based techniques like random search and grid search are used as samplers. But we point out three limitations in using these techniques. First, they are passive samplers, which do not use the feedback of previous results in the sampling process. Second, the variables to be sampled may have constraints that are often not included by existing approaches. Third, they do not balance the tradeoff between exploration and exploitation, which we hypothesize is needed for better coverage of the search space. To address these limitations, we present a scene generation approach with two samplers called Random Neighborhood Search (RNS) and Guided Bayesian Optimization (GBO). These samplers extend the conventional random search and Bayesian Optimization search with the limitation points. Also, to facilitate the samplers, we use a risk-based metric that evaluates how risky the scene was for the system. We demonstrate our approach using an Autonomous Vehicle example in CARLA simulation. To evaluate our samplers, we compared them against the baselines of random search, grid search, and Halton sequence search. Our samplers of RNS and GBO sampled a higher percentage of high-risk scenes of 83\% and 92\%, compared to 56\% 66\% and 71\% of the grid, random and Halton samplers, respectively. 


 

% to identify shifts in the operating environment and estimate the likelihood of system failures.

% Data from these high-risk conditions is often not available during training. Also,

 

% samplers of RNS and GBO sampled a higher percentage of high-risk scenes of 83\% and 92\%, compared to 56\% of the traditional grid search sampler. 

 

% sequential search-based samplers that can efficiently generate high-risk simulation scenes. The two sampling approaches are Random Neighborhood Search (RNS) and Guided Bayesian Optimization (GBO). These samplers employ a sequential search strategy in which they use the system's earlier performances for strategically sampling the variables for the next scene. To facilitate the samplers, we use a novel performance metric called the safety score, which evaluates how risky the scene was for the system. We demonstrate our approach using an Autonomous Vehicle case study in CARLA simulation. Our samplers of RNS and GBO sampled a higher percentage of high-risk scenes of 83\% and 92\%, compared to 56\% of the traditional grid search sampler. 






% We also show that our samplers help reveal the critical risky scenes, which are often missed by the traditional samplers.

% So, it is critical to find these high-risk scenes for designing the safety components and periodically updating them to incorporate the knowledge of these high-risk scenes, which can improve the system's robustness.


\end{abstract}

\begin{IEEEkeywords}
Cyber-Physical Systems, Dynamic Assurance, Dynamic Risk, High-risk Scene, Bow-Tie Models, Hazards
\end{IEEEkeywords}

==> Accepted/individual-sections/approach.tex <==
\section{Proposed Approach}
\label{sec:approach}
Overview of our approach is illustrated in \cref{fig:workflow}, and it consists of the following three broad components: (1) A scene generation approach designed using a \acl{sdl}. (2) A risk-based metric that is used to score the generated scenes. (3) The proposed sampling approaches called \acl{rns} and \acl{gbo}. We describe these components in detail below.  

\subsection{Scene Generation}
\label{sec:scene_generation}
We have designed a probabilistic scene generation language to generate scenes. The language includes a \acl{sdl} (SDL) integrated with probabilistic samplers to sample scenes over different scene variables introduced in \cref{sec:ps}. The \ac{sdl} has two components. (a) \textit{grammar}, which consists of a set of rules required to define the scene concepts in the meta-language. (2) \textit{meta-model}, which defines the concept of a scene using scene variables and their distribution ranges. In this setup, a scene $s$ = \{$e_1$,$e_2$,...,$e_i$\} is a collection of entities, where each entity is a three tuple $<s_v,v_d,v_c>$ of the scene variables $s_v$, distribution properties $v_d$ (e.g., distribution type, ranges) and variable constraints $v_c$. The language is designed using the textX \cite{dejanovic2017textx} meta-language. The language also has an interpreter to generate the scene artifact files and run the simulator. In addition, the interpreter abstracts the complexity of the language from the user by providing a scene specification file with scene variables and samplers that can be chosen to generate different scenes. The scene generation approach is illustrated in \cref{fig:workflow}.  


\subsection{Scoring Function}
\label{sec:scoring}
% We have designed a risk-based metric called the \textit{Risk Score} ($S_{Risk}$) to score the sampled scene. This score is a weighted combination of two utility functions $S_{Risk} =  w_1 \cdot RS + w_2 \cdot IS$. The utility functions are. (1) \textit{\ac{resonate} Score} ($RS$), which measures the system's dynamic risk in the scene using the likelihood hazard rates measured by \ac{resonate} discussed in \cref{sec:risk_estimation}. (2) \textit{Infraction Score} ($IS$), which measures the actual infractions (e.g., running a stop light) performed by the system. In this work, we used equal weights $w_1$ = $w_2$ = 1 for both these utility functions. We did this to ensure that both the estimated risk and the actual risk caused by actual infractions are equally weighted in the subsequently sampled scenes. 

We have designed a risk-based metric called the \textit{Risk Score} ($S_{Risk}$) to score the sampled scene. This score is a weighted combination of two utility functions and is computed as $S_{Risk} =  w_1 \cdot RS + w_2 \cdot IS$. The utility functions are. (1) \textit{\ac{resonate} Score} ($RS$), which measures the system's dynamic risk in the scene using the likelihood hazard rates measured by \ac{resonate} discussed in \cref{sec:risk_estimation}. (2) \textit{Infraction Score} ($IS$), which measures the actual infractions (e.g., running a stop light) performed by the system. In this work, we used equal weights $w_1$ = $w_2$ = 1 for both these utility functions. We did this to ensure that both the estimated risk and the actual risk caused by infractions are equally weighted in the subsequently sampled scenes. 



% \begin{equation}
% \label{eqn:risk_score}
%     S_{Risk} =  w_1 \cdot RS + w_2 \cdot IS
% \end{equation}


% In future work, we will vary these weights to see the impact on the kind of scenes that will be sampled. 

% The metric evaluates a scene based on the risk it poses to the system's safe operation. However, instead of only using the operational system risk that is estimated using the likelihood failure rates predicted by \ac{resonate}, we also include the actual system infractions in scoring a scene. So, the scoring function is a sum of the \textit{\ac{resonate} Score} ($RS$) and the \textit{Infraction Score} ($IS$). 

% Rather denote that there are two utility functions. One that measures RS and the other that measures IS. The overall utility function that you seek to maximize in the new samples is a weighted combination of both. You chose to provide same weight to both. This ensures that the scenes with both perceived risk and actual risks are equally weighted and identified in the future samples. In future it will be an interesting experiment to see what happens if you change these weights.

% While $RS$ provides the average likelihood of the system consequence across the scene, $IS$ provides the actual system infractions. 

% \begin{equation}
% \label{eqn:safe_score}
%     S_{Risk} =   \ac{resonate} \; Score + Infraction \; Score
% \end{equation}
% uses the design-time probabilities of the \ac{btd} event along with runtime measurements from monitors like anomaly detectors and \ac{ood} detector to

\subsubsection{\ac{resonate} Score ($RS$)} Measures the average risk of the system's consequence across the scene. To compute this score, we leverage the \ac{resonate}~\cite{hartsell2021resonate} risk estimator which estimates the dynamic hazard rate $\lambda$ at every time step. The hazard rates are averaged across the scene using $\frac{\int_{T_1}^{T_2} \lambda \,dt}{T_2-T_1}$, where $\lambda$ is the estimated hazard rate and $T_1$, $T_2$ are the start and end time of the scene, to compute the system's dynamic risk or the \ac{resonate} score. In this work, our simulations are typically $1$ minute long, so $T_1$=0 and $T_2$=1 are used in the calculations.

\subsubsection{Infraction Score ($IS$)} Measures the system's actual infractions in the simulator. This score can include a variety of infractions like route deviation, lane violation, and traffic rule violation. These infractions ($I_k$) can be weighted ($w_k$) according to their severity and later summed together to compute the infraction score $IS$ = $\sum_{k=1}^{n} w_k \cdot I_k$. To illustrate, the infraction score for the \ac{av} case study was computed as $IS = 0.7 \cdot I_S + 0.8 \cdot I_R + I_{RD}$. Where $I_S$ is running a stop sign infraction, $I_R$ is running a red-light infraction, and $I_{RD}$ is the deviation in the route taken by the \ac{av}.  


% \begin{equation}
%     Infraction \; Score = \sum_{k=1}^{n} w_k \cdot I_k
% \label{eqn:driving_score}
% \end{equation}


% Finally, we compute $S_{Risk}$ using these two scores.

% For the \ac{av} case study, we have used the weighted sum of the Infraction penalties ($I$) and the Route Deviation ($I_{RD}$) metrics as $IS = 0.7 \cdot I_S + 0.8 \cdot I_R + I_{RD}$.

% An example of these infractions for two different scenes is shown in \cref{fig:hazard_rate}.  

% \begin{figure}[t]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/hazard-rate.pdf}
%  \caption{The estimated collision rate for two test scenes. (Top) Scene1 - A scene with two camera faults. The average collision rate across the scene was $0.4$ and the infraction score was $0$ (Bottom) Scene2 - A scene with adverse brightness. The average collision rate across the scene was $0.69$ and the infraction score was $0.15$.}
%  \label{fig:hazard_rate}
%   \vspace{-0.15in}
% \end{figure}

Given these scores, we compute $S_{Risk}$ for the scene. Further, the scene is classified to be high-risk if $S_{Risk} - \delta$ $>$ 0. Where $\delta$ is the risk threshold computed across the previously encountered calibration scenes. Considering these scenes are sampled from the same underlying distribution, we 
select a simple threshold at the $95^{th}$ percentile ($2$ standard deviations) of $S_{Risk}$ for every scene in the calibration set. 

% Now, a scene with $S_{Risk}$ $>$ $\delta$ is classified to be high-risk. $\delta$ is the risk threshold computed across the previously encountered calibration scenes. Considering these scenes are sampled from the same underlying distribution, we select a simple threshold at the $95^{th}$ percentile ($2$ standard deviations) of $S_{Risk}$ for every scene in the calibration set. 

% Now, for classifying the scene as high-risk, we calculate a risk score threshold $\delta$ across all the previously encountered scenes. This threshold is calculated across a part of the calibration set, which is not used for designing the risk-estimator. This set includes scenes with sensor faults and adverse brightness along with the normal scenes from training. Now, as these scenes are sampled from the same distribution, we use $2$ standard deviations ($\mu$ + $2\cdot\delta$) of the $S_{Risk}$ score across the calibration set as the threshold. In our setup, any scene that has $S_{Risk}$ $\geq$ $\delta$ is classified to be of high-risk.

\input{results/rns}

\subsection{Sampling Approaches}
\label{sec:samplers}
We present two samplers called the \acl{rns} and \acl{gbo}, which are extensions of the conventional random and \ac{bo} search. The extensions are. (1) \textit{active sampling}, we use a feedback loop of previous simulation results to sample the next scene variables. (2) \textit{constraints-based search}, we create sampling constraints $\mathcal{SC}$ to add constraints on the scene variables. \cref{Table:constraints} shows the constraints that we applied for an \ac{av} case study. (3) \textit{exploration vs. exploitation trade-off}, we introduce explicit hyper-parameters to balance the strategies.


% \input{results/sampling_rules}


\subsubsection{Random Neighborhood Sampler (RNS)}
This sampler extends the conventional random search by including the kd-tree nearest neighborhood search algorithm~\cite{friedman1975algorithm}. With this extension, we aim to add the missing exploitation capability to random search. Briefly, the approach works as follows. It initially explores a scene through random sampling and then exploits the area around the explored scene using the sampling constraints and the nearest neighbor search. \cref{algo:rns} illustrates the steps involved, and it works as follows. 

\textit{First}, the algorithm explores the search space $\mathcal{D}$ by randomly sampling the scene variables $s_v$ from their respective distributions $V_D$. These randomly selected variables are used to generate the scene artifact files, run the simulator and compute the risk score $S_{Risk}$ for the scene. The randomly generated scene is represented as $R$ in \cref{fig:workflow}.

\textit{Second}, if the $S_{Risk}$ $<$ $\delta$, the simulation run statistics are stored, and the scene variables are again randomly sampled from the search space $\mathcal{D}$. However, if the $S_{Risk}$ $>$ $\delta$, the neighborhood around the randomly sampled scene $R$ is exploited to generate more scenes. For this, we create a bounded region $\mathcal{B}$ around $R$ using the sampling constraints $\mathcal{SC}$ shown in \cref{Table:constraints}.


% For this, we use the sampling constraints $\mathcal{SC}$ shown in \cref{Table:constraints}. These constraints will create a bounded region $\mathcal{B}$ around $R$ from which the subsequent scene variables are randomly sampled. 

\textit{Third}, the algorithm uses the kd-tree nearest neighborhood search to find if there are at least $k$ scenes generated in the neighborhood of the explored scene $R$. That is, it checks if $R$ has at least $k$ similar scenes in $\mathcal{E}$. To measure the similarity, we use the $l_2$ distance metric $(d(x,R) = ||x - R||_2)$ and identify the similar scenes as $N = \{\forall s \in \mathcal{E}| d(R,s_i) < \tau \}$. Where $R$ is the currently sampled scene and $s_i$ are scenes in the previously explored list $\mathcal{E}$. This step returns a list of neighbors whose distances to $R$ are smaller than a threshold $\tau$.  If the number of the neighbors $N$ $\geq$ $k$, the search around $R$ is stopped. Then,  step1 is performed to randomly explore a new scene in the entire search space $\mathcal{D}$. However, if $N$ $\leq$ $k$, then the search around $R$ is continued. In this sampler, $k$ is the hyperparameter used to control the exploitation.


% using the following equation. 

% \begin{equation}
% \label{eqn:distance}
%     N = \{\forall s \in \mathcal{E}| d(R,s_i) < \tau \}
% \end{equation}

\input{results/bo}

\begin{figure*}[t]
 \centering
 \includegraphics[width=0.82\textwidth]{figures/simulation-scene4.pdf}
 \caption{Screenshots of different scenes generated for the CARLA \ac{av} case study. The description of these scenes are provided below the images.}
 \label{fig:scenes}
\vspace{-0.1in}
\end{figure*}


\textbf{Limitation:} Although the sampler can both explore and exploit the search space, the exploration is performed uninformed without strategic knowledge about the search space. This could result in high-risk regions of the search space left unexplored.

\subsubsection{Guided Bayesian Optimization (GBO)}
\label{sec:gbo_sampler}
The uninformed exploration of \ac{rns} is addressed by this sampler, which is an extension to the conventional \acl{bo}. To perform informed exploration and active sampling, the algorithm has two components. (1) Probability function model that is fitted across all the previously explored variables. This feedback allows the model to learn the region of the search space that has large uncertainty that will return a higher objective value. A \ac{gp} model is most used to fit the function. (2) Acquisition function that strategically finds the succeeding variables, which will optimize the objective function. We use the \ac{ucb}~\cite{auer2002using} acquisition function that provides the $\beta$ hyperparameter to control the exploration vs. exploitation trade-off (See \cref{eqn:ucb}). We also include the sampling constraints to the acquisition function to restrict the region in which it looks for the next sampling variables. \cref{algo:bo} shows the operation of the \ac{gbo} sampler, which is discussed below. 

\textit{First}, the \ac{gp} model with properties $\mu$[0] and $\sigma$[0] is initialized for first k iterations. During these iterations, the scene variables $s_v$ are randomly sampled from the input search space $\mathcal{D}$. These randomly sampled variables are used to generate scene artifact files and run the simulation. Then, $S_{Risk}$ is computed and added to the exploration list $\mathcal{E}$ along with the sampled variables. After the k initial iterations, the initialized \ac{gp} model is fitted across all the entries in $\mathcal{E}$ to calculate new posterior distribution $f(x_n)$ with updated $\mu$[$x_n$] and $\sigma$[$x_n$]. 

% . Then, the marginalization property of the \ac{gp} model allows for the calculation of a new posterior distribution $f(x_n)$ with an updated posterior mean $\mu$[$x_n$] and $\sigma$[$x_n$]. 

\textit{Second}, the algorithm uses the sampling constraints $\mathcal{SC}$ to create a smaller search space $\mathcal{B}$ in which the acquisition function will sample the succeeding variables. The updated posterior distribution and the bounded search space created by the sampling constraints are used by an acquisition function to strategically select the subsequent scene variables that will optimize $S_{Risk}$. In this work, we use the \ac{ucb} \cite{auer2002using} as the acquisition function, which is given below. 
 
\begin{equation}
\label{eqn:ucb}
    x_{n+1} = \argmax\limits_{x \in \mathcal{D}}\mu[x_n] + \beta^{1/2} \cdot \sigma[x_n]
\end{equation}

Where $x_{n+1}$ are the newly selected variables that have the largest \ac{ucb}. $\mu[x_n]$ and $\sigma[x_n]$ are the properties of the updated \ac{gp} model. $\beta$ is a parameter that allows for exploitation and exploration tradeoff. A larger value of $\beta$ allows for higher exploration, and a lower value allows for exploitation. So, $\beta$ needs to be carefully selected for optimizing the two strategies. The newly selected variables are used to run the simulation and compute $S_{Risk}$, which is added to the list $\mathcal{E}$ along with the selected variables. The steps of the algorithm are repeated for a specified number of iterations $t$.  

\textbf{Limitation:} The sampler has two problems that arise because of using the \ac{gp} model. (a) Cold-start, which requires the model to be trained from scratch each time the sampler is used. This increases the sampling time. To address this, we use the knowledge of randomly sampled scenes from the previous runs to ``warm start" the search process. (b) Scalability, the \ac{gp} model suffers from a cubic time complexity~\cite{liu2020gaussian}, which limits its applicability to a large number of executions. To address this, we will use a scalable \ac{gp} model in the future.  





==> Accepted/individual-sections/background.tex <==
\section{Background}
\label{sec:background}
% In this section, we introduce the Dynamic Assurance topics that are required to understand our approach.
% - explain what you assume about system design procedures.
% - background on dynamic assurance.
% - explain BTD


\subsection{System Design Procedures}
We assume that the \ac{cps} undergoes design, training, and deployment activities categorized into four steps: (1) \textit{Design Phase}, which involves system analysis, hazard analysis, and Assurance Case construction. (2) \textit{Training Phase}, which involves collecting training scenes and training the \acp{lec} on these scenes. (3) \textit{Calibration Phase}, which involves calibrating anomaly detectors, \ac{ood} detectors ~\cite{cai2020real,sundar2020out} and dynamic assurance monitors (\cref{sec:risk_estimation}) for estimating the system risk. Calibration requires curating a \textit{calibration set} that includes scenes with sensor faults and adverse weather in addition to the training scenes. (4) \textit{Testing Phase}, which involves generating high-risk test scenes for testing the trained system. 

% and identifying the operating conditions in which they fail.

%We briefly describe these steps and expectations below.

In particular, the design phase is important because it consists of gathering and documenting information about the system's top-level goals, requirements, system operating conditions, and system faults. It also includes designing the system models including, architecture model (e.g., \cref{fig:sys-model}), and system function breakdown.  Thereafter, we assume that the designers perform \textit{Hazard Analysis}, which involves identifying the hazards to the system that will result in a system consequence. The system could have a collection of hazards $\{H_1, H_2,\cdots, H_n\}$ stemming from its operation, functioning, software components, and hardware components. Any of these hazards in a given condition can result in a system consequence. This enables creation of \ac{btd}~\cite{ferdous2013analyzing}, a model describing the chain of events $t_i \rightarrow b_p \rightarrow e_{top} \rightarrow b_m \rightarrow c_i$, where $t_i$ are system threats, $b_p$ are preventive barriers, $e_{top}$ is a top event, $b_m$ is a mitigation barrier, and $c_i$ is a system consequence. Fig \ref{fig:btd} describes the operational hazard of ``roadway obstruction'' for the \ac{av} case study (\cref{fig:sys-model}). The \ac{btd} has two system threats: vehicles (T1) and pedestrians (T2) in the path of the ego vehicle. These threats can escalate to become a top event (TOP) if preventive barriers of $B1$ and $B2$ are not introduced. The performance of the perception \ac{lec} is used as the barrier. If the perception LEC fails, then the roadway hazard can become a safety consequence $C1$ if not mitigated by a barrier of $B3$, the emergency braking system.  During the design, these hazard analyses are used to create assurance cases~\cite{bishop2000methodology}, showing that the top-level goals of the system are satisfied. Further, such hazard diagrams enable the system to be dynamically monitored for the likelihood of failures through a technique called dynamic assurance. 

     
 \iffalse   
 The \textbf{training} phase consists of developing the  \ac{lec}s. The 
    \item \textbf{Training Phase}: We assume the training phase consists of the data collection and the design and training of the \ac{lec}s. These components are mostly deep neural networks that are often trained through supervised learning~\cite{hastie2009overview} or reinforcement learning~\cite{sutton2018reinforcement}. The training process is often cumbersome with several hyperparameters to tune (e.g., model architecture layers, training epochs, batch size). Tool-chains like ALC~\cite{hartsell2019model} assist the hyperparameter selection and training process. 
    
    % \textcolor{red}{please put citations - like our ALC papers}
    
   
    \item \textbf{Calibration Phase} : We assume the calibration phase consists of designing and calibrating runtime monitors for dynamic assurance.
    %Along with conventional anomaly detectors for detecting software and hardware anomalies, it is required to consider the uncertainties of \ac{lec}s for \acl{ood} scenes.
    Detecting the \ac{ood} data problem requires designing complex anomaly detectors called \ac{ood} detectors or assurance monitors~\cite{cai2020real,sundar2020out}. Finally, estimating the system risk also requires designing risk estimators~\cite{hartsell2021resonate} (e.g. \cref{sec:risk_estimation}). %These monitors are trained and calibrated using the training data.   
    
    % \textcolor{red}{put citations of xenofon, penn and berkley and other papers}
    
   % Describe OOD detectors and other monitors trained
    \item \textbf{Operational Phase}: We assume at runtime, the trained \ac{lec} with the calibrated runtime monitors are used for operating the system. At each time step, the \ac{lec} predicts the control actions for the system, and the runtime monitors detect any outliers in the sensor measurements or changes in the operating conditions. The results from these runtime monitors can be used to assess the dynamic risk to the system using a dynamic assurance framework. 
    %    are often used for high-level controller selection~\cite{zakharov2015performance} based upon  
    
    % During the runtime, dynamic assurance framework is deployed -- summarize
% \end{enumerate}
\fi
%\textbf{Operational Phases}:We classify the design, training, and deployment activities into $4$ phases as shown in \cref{fig:workflow}. They are. (1) \textit{Design Phase}, which involves system analysis, hazard analysis, and Assurance Case construction. (2) \textit{Training Phase}, which involves collecting training scenes and training the \ac{lec} controllers and the anomaly detectors on these scenes. (3) \textit{Calibration Phase}, which involves designing and calibrating the risk estimator. Estimating the system risk requires curating a calibration set that includes scenes with sensor faults and adverse operating conditions in addition to the training scenes. (4) \textit{Testing Phase}, which involves generating high-risk test scenes for testing the trained system.

% The system can have several top level goals adhering to different properties of the system like safety, security, functional, etc.
\iffalse
\textbf{1) System Analysis} involves gathering and documenting information about the system's top-level goals, requirements, system's operating conditions, and system faults. It also includes designing the system models including, architecture model (e.g., \cref{fig:sys-model}), and system function breakdown. 

\textbf{2) Hazard Analysis} involves identifying the hazards to the system that will result in a system consequence. The system could have a collection of hazards $\{H_1, H_2,\cdots, H_n\}$ stemming from its operation, functioning, software components, hardware components, etc. Any of these hazards in a given condition can result in a system consequence. A \ac{btd} \textcolor{red}{cite BTD} is a graphical structure that is often designed to analyze the hazard propagation and identify the possible control strategies to prevent the hazard from failing the system. The \ac{btd} can be represented as a chain of events $t_i \rightarrow b_p \rightarrow e_{top} \rightarrow b_m \rightarrow c_i$. Where, $t_i$ are system threats, $b_p$ are preventive barriers, $e_{top}$ is a top event, $b_m$ is a mitigation barrier, and $c_i$ is a system consequence. To explain these events, consider the \ac{btd} (See \cref{fig:btd}) for an operational hazard of ``roadway obstruction" for an \ac{av} case study that is introduced later in \cref{sec:casestudy}. To explain the \ac{btd}, it has two system threats of vehicles (T1) and pedestrians (T2) in the travel paths, which is derived from hazard analysis. Now, these threats can escalate to become a top event (TOP) if preventive barriers of $B1$ and $B2$ are not introduced. In this case, the performance of the \ac{lec} is used as the barrier. Next, the top event could escalate to become a consequence not mitigated by a barrier of $B3$. In this example, the performance of AEBS in emergency braking is selected as the barrier. 

\textbf{3) Assurance Case Construction} involves using the system and hazard analysis information to construct an assurance case~\cite{bishop2000methodology}, which can argue using the available system evidence that the top-level goals of the system are satisfied.   

% to handle dynamically changing operating conditions in which these systems operate
\fi
\subsection{ReSonAte}
\label{sec:risk_estimation}
%Design-time information is  used to assure the system properties (e.g., safety, security) at runtime. However, 

%Static assurance cases  are not very accurate because the system hazards can be dependent on the operating conditions and the system state~\cite{denney2015dynamic}. 
%For example, a hazard (e.g., camera blur) that is of high consequence in one operating condition (e.g., night) can have a low consequence in the other (e.g., day). To capture this,
%The dynamic assurance approach  uses runtime measurements in addition to the static assurance cases to estimate the ``system's dynamic risk". %
%\ac{resonate}~\cite{hartsell2021resonate} is an example of dynamic assurance framework.



%with the design-time information is required. Our approach to dynamic assurance is to estimate the ``system's dynamic risk". 
%\textbf{ReSonAte:} To perform dynamic risk estimation, we leverage our previously developed tool called \ac{resonate}~\cite{hartsell2021resonate}. The tool uses the 
%\ac{btd} to estimate the dynamic hazard rate $\lambda$ for every hazard that is identified in the design phase. The hazard rate can be used to compute the likelihood of the hazard occurrence in a given time unit $1-e^{-\lambda \cdot t}$, where $\lambda$ is the estimated hazard rate, and $t$ is the duration..
%The likelihood of different hazards contributes to the system's risk. 

% In this setup, we consider the likelihood of different hazards to be independent.
 
% The system can have several hazard rates stemming from different hazardous failures. These rates put together constitute the system's risk. For estimating $\lambda$, \ac{resonate} uses a hazard propagation structure called \ac{btd}. Designing the \ac{btd} is a design-time activity, which begins with hazard analysis, which includes identifying the events to the system like Threats (T), which may lead the system into a hazard (H), and the possible barriers (B) to prevent the hazard from propagating into a consequence. These hazard events are used to design a \ac{btd}, which is often used to visualize hazard propagation, identify control strategies, and estimate the system's risk.  

To perform dynamic assurance, we leverage our previously developed tool called \ac{resonate} ~\cite{hartsell2021resonate}, which uses an augmented \ac{btd} (derived from the hazard analysis). The augmentation adds various event probabilities for each causal chain, conditioned on the state of the system and the environment, including sensor failures, actuator failures, and output of \ac{ood} detectors and environmental conditions. Specifically, it requires estimation of the (a) the conditional probability of the barrier's success in each state $(f_b(x=B_i),s)$, and (b) the frequency of occurrence of a threat $f_e(T_i,s)$ in each state. These conditional relationships must be inferred from data and are often inferred by using the observation of system's and barrier's performance across various scenes. For this, we use the calibration set collected using a grid sampler, where we select the conditions affecting the barrier and generate scenes around it. The estimated probabilities are stored in \acp{lut} as illustrated in \cref{fig:btd}. At runtime, the \acp{lut} is used to identify the current context and then identify the hazard rate for the consequence ($\lambda$). The hazard rate can then be used to compute the likelihood of the hazard occurrence in each time unit $1-e^{-\lambda \cdot t}$, where $\lambda$ is the estimated hazard rate, and $t$ is the duration. 

 
%The hazard rate is estimated using a \ac{btd}, and it requires calculating the probabilities of the different events in the \ac{btd}. The probabilities that are of interest are. (a) the conditional probability of the barrier's success in each state $(f_b(x=B_i),s)$. and (b) the frequency of occurrence of a threat $f_e(T_i,s)$ in each state. This term gives the expected frequency of threat in units of the expected number of occurrences in a given time interval. Also, it is important to note that these probabilities may be conditionally dependent on the system's state ($s$) including sensor failures, system failure modes, anomaly detectors, and environmental conditions. To model conditional dependence, we need to identify the conditions relevant to the barriers. These conditional relationships must be inferred from data. For this, we generate a calibration set using a grid sampler, where we select the conditions affecting the barrier and generate scenes around it. The estimated probabilities are stored in \acp{lut} as illustrated in \cref{fig:btd}, and their calculations are discussed in \cref{sec:evaluation}. 

%Now, these probabilities are used with runtime measurements from detectors to estimate the dynamic hazard rate and the system's dynamic risk. We refer to this dynamic risk as to the \ac{resonate} score in this paper. Along with conventional anomaly detectors to identify outliers in sensor measurements and software components, it is required to consider the uncertainties introduced by the \ac{lec}s because of the \acl{ood} conditions. This requires designing complex anomaly detectors called \ac{ood} detectors~\cite{sundar2020out}. 

% Now, estimating this score requires designing anomaly detectors to identify outliers in sensor measurements and software components.  Also, it is required to consider the uncertainties introduced by the \ac{lec}s because of the \acl{ood} conditions. This requires designing complex anomaly detectors called \ac{ood} detectors~\cite{sundar2020out}. 





% \subsection{CPS operational Phases}
% To perform dynamic assurance of autonomous \ac{cps}, we classify the design, training and deployment activities into the following phases. (1) \textit{Design Phase} involves system analysis, hazard analysis and construction of an Assurance Case. (2) \textit{Training Phase} involves collecting training scenes and training the \ac{lec} controllers and the anomaly detectors on these scenes. (3) \textit{Calibration Phase} involves designing and calibrating the risk estimator. Estimating the system risk requires curating a calibration set that includes scenes with sensor faults and adverse operating conditions in addition to the normal training scenes. (4) \textit{Testing Phase} involves generating high-risk test scenes for testing the trained system.

% which the system has high operational risk and is susceptible to fail. 

% designing and modeling the system, identifying the system operating conditions, identifying the system hazards, sensor faults, and finally designing an Assurance Case.


% using the proposed samplers to generate high-risk scenes for testing the trained \ac{lec} and the safety components. In the future, we will use the generated high-risk scenes to iteratively update the controller and the safety components. 



==> Accepted/individual-sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented a scene generation approach that integrates a \acl{sdl} with two samplers and a risk-based scoring function for generating high-risk scenes. The proposed samplers are \acl{rns} and \acl{gbo}. These samplers are based on the conventional random and \ac{bo} search techniques, and we add capabilities of active sampling, constraint-based sampling, and balancing the exploration vs. exploitation to guide them towards sampling clusters of high-risk scenes. We applied these samplers to an \ac{av} case study. Our evaluations show that the proposed samplers could sample a higher number of high-risk scenes that could be clustered into a higher number of clusters as compared to the conventional baselines. 

\textbf{Acknowledgement}: This work was supported by the DARPA Assured Autonomy project and Air Force Research Laboratory. 


% Also, we have designed a novel scoring function to score the scenes and guide the samplers. We demonstrate this workflow for an \ac{av} example in CARLA simulation. Our samplers outperformed the baselines in terms of the total risk scenes, diversity, and search time metrics.

% extend the conventional random search and \ac{bo} search with additional capabilities

% Future extensions of the approach include. (1) \acl{rl} sampler to generate a sequence of scenes that pose high-risk to the system, (2) perform continual learning of the models as smaller batches of high-risk scenes rather than a single update at the end of testing phase. 

% Further, the high-risk scenes generated by the samplers are used to periodically update the system models to avoid concept drift and model staleness.

==> Accepted/individual-sections/evaluation.tex <==


% \footnote{\label{github}source code to replicate the CARLA experiments can be found at \url{https://github.com/Shreyasramakrishna90/Risk-Aware-Scene-Generation}}

\section{Evaluation}
\label{sec:evaluation}
We evaluate our approach using an \ac{av} example in CARLA simulator~\cite{dosovitskiy2017carla}. The experiments were performed on a desktop computer with AMD Ryzen Threadripper 16-Core Processor, 4 NVIDIA Titan Xp GPU's and 128 GiB RAM memory.



\subsection{\ac{av} Case Study}
\label{sec:casestudy}

Our testbed is an \ac{av} that is needed to navigate an urban town with adverse weather conditions and sensor faults while avoiding collisions with vehicles and pedestrians in its travel path. For this setup, we leverage the CARLA autonomous driving challenge~\cite{carla-challenge}, which in addition to complex driving scenarios, also provides individual metrics to measure the \ac{av}'s infractions. The details of \ac{av} setup are discussed below. 


% in the CARLA autonomous driving challenge~\cite{carla-challenge}. The \ac{av} is needed to navigate a town with adverse weather conditions and sensor faults while avoiding collisions with vehicles and pedestrians in its travel path. The simulator also offers individual metrics to measure the \ac{av}'s infractions. The details of \ac{av} setup are discussed below.  

\subsubsection{System Model} The system block diagram of the \ac{av} is shown in \cref{fig:sys-model}. It uses a total of $9$ sensors including, three forward-looking cameras, two radars, an \ac{imu}, a \ac{gps}, and a speedometer. It has a \ac{lec} based navigation controller, which is adapted from Chen et al.~\cite{chen2020learning}. This controller uses a navigation planner that takes the waypoint information from the scene artifact file generated by our scene generation approach and divides the distance between the waypoints into smaller position targets. Then, it uses the \ac{gps} and \ac{imu} sensors to get the vehicle's current position and the next position to reach. Next, the position information is fed into a velocity planner to compute the vehicle's desired speed. The desired speed and camera images are fed into a perception \ac{lec}, which predicts the throttle and steering angle errors. These signals are sent to PID controllers to compute the throttle, brake, and steer control signals. Besides the \ac{lec}, there is also an \ac{aebs}, which uses the radar estimated object distance ($r_d$) with the vehicle's current speed to compute a ``safe braking distance" ($b_d$). If $r_d \leq b_d$, a brake alarm is issued. The alarm overrides the throttle signals from the \ac{lec}. Finally, these control signals are sent to the simulator. 

\subsubsection{System Operational Phases} The \ac{av} is operated in the following phases. In the \textit{Design phase}, we designed the system model in \cref{fig:sys-model}. We then performed hazard analysis to identify the operational threats to the \ac{av}. Next, we identified sensor faults (camera blur and occlusion) that affected the \ac{av}'s performance. In the \textit{Training phase} we used the \ac{av}'s autopilot controller to collect data for training the perception \ac{lec} using the training procedure discussed in~\cite{chen2020learning}. In the \textit{Calibration phase}, we calibrate the anomaly detector, \ac{ood} detector and the \ac{resonate} risk estimator. For risk estimation, we curated a calibration set that included scenes from the training set and additional scenes with sensor faults and adverse weather conditions, collected using a grid sampler. Finally, in the \textit{Testing Phase}, the trained \ac{lec} and the monitors are tasked to operate in $250$ test scenes generated by the proposed samplers. These scenes included varying the weather conditions (cloud (C), precipitation (P)), time-of-day (T), traffic densities (TD), road segments (RS), and sensor faults (F). The distribution ranges of these scene variables and their sampling constraints are listed in \cref{Table:constraints} and are discussed in \cref{sec:ps}. \cref{fig:scenes} illustrates the screenshots of a few test scenes.



% \begin{minipage}[!htb]{0.95\columnwidth}
% \centering
% \begin{minipage}{0.25\columnwidth}
% \begin{figure}[H]
%         \input{results/scene}
% \end{figure}
% \end{minipage}
% \hspace{0.28\columnwidth}
% \centering
% \begin{minipage}{0.4\columnwidth}
% \begin{figure}[H]
%         \input{results/faults}
% \end{figure}
% \end{minipage}
% \footnotesize
% \centering
% % \setlength{\abovecaptionskip}{2pt}
% \captionof{figure}{(left) Simulation Variables and their distribution ranges. (right) types of sensor faults considered in these scenes.}
% \label{Table:variables}
% \vspace{0.15in}
% \end{minipage}


% \subsubsection{Operating Scenes} As illustrated in \cref{fig:scenes}, our scenes included varying the weather conditions (cloud (C), precipitation (P)), time-of-day (T), traffic densities (TD), road segments (RS), and sensor faults (F). The distribution ranges of these scene variables and their sampling constraints are listed in \cref{Table:constraints} and is discussed in \cref{sec:ps}. 

% To remind, the road segment has constraints on the distance between two consecutive waypoints. Also, the weather variables have constraints on how much their values can change between consecutive scenes. Traffic density is a special case that had constraints on its values, and it is also dependent on the type of road segments. Finally, camera blur and occlusion are the two faults that are injected into the three cameras on the vehicle.   


% \cref{fig:sampling-rules} while sampling these variables. 

% The structural variables of road segments and traffic density had constraints that were defined by the CARLA map. For example, the sub-rages for traffic were selected based on the vehicle's location (e.g., crossroads, intersections). The temporal variables had the constraint $n$ (see \cref{fig:sampling-rules}) on the rate at which its value changes. For this example, the value of $n$ = 5 was chosen. In addition, \cref{Table:variables} shows the sensor faults that we synthetically injected into the vehicle. 

% Also, we add Gaussian noise to the distances returned by the radar. 


% \begin{figure}[!t]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/scene-variables.pdf}
%  \caption{(left) Simulation Variables and their distribution ranges. (right) types of sensor faults considered in these scenes.}
% \label{Table:variables}
% \vspace{-0.1in}
% \end{figure}


\subsubsection{Detectors} 
\label{sec:safety_components}
% To augment safety into the vehicle, we equipped it with several anomaly detectors and an \ac{ood} detector. 
To detect camera-related faults such as blurred images and occluded images, each of the three cameras is equipped with OpenCV based blur detector and occlusion detector. The blur detector uses the variance of the Laplacian operator~\cite{pech2000diatom} to measure the blur level in the images. A high variance shows that the image is not blurred, and low variance ($<50$) shows the image is blurred. The occlusion detector is designed to identify large blobs of continuous black image pixels. In our setup, if an image has connected black pixels $>10\%$, then the image is said to be occluded, otherwise, it is not. The blur detectors and the occlusion detectors had an F1-score of 97\% and 98\% on the calibration set. 

% We empirically selected these thresholds based on the calibration set.

In addition, we designed a reconstruction-based $\beta$-VAE \ac{ood} detector~\cite{sundar2020out} to identify shifts in the operating scenes. The detector model has four convolutional layers $16/32/64/128$ with (3x3) filters and (2x2) max-pooling followed by four fully connected layers with $2048$, $1000$, and $250$ neurons. It also has a symmetric deconvolutional decoder structure and hyperparameters of $\beta$=1.2 and latent space=$100$. We trained the model for $150$ epochs using the $6000$ center camera images. We tested it by synthetically introducing brightness into the training images. For these images, the detector had an F1-score of 98\%. At runtime, the reconstruction mean squared error of the detector is used with Inductive Conformal Prediction \cite{shafer2008tutorial} and power martingale \cite{fedorova2012plug} to compute a martingale value. We use the martingale value with a threshold of $20$, which was empirically selected for \ac{ood} detection. 

\begin{figure*}[t]
 \centering
 \includegraphics[width=0.9\textwidth]{figures/sampler-plots2.pdf}
 \caption{Comparison of the $250$ scenes sampled by the different samplers. While random and Halton samplers only explore the space, grid sampler only exploits. Our samplers balance the exploration vs. exploitation, which is evident from the dense scene clusters in different regions of the search space.}
 \label{fig:sampler_3d}
\vspace{-0.1in}
\end{figure*}


\subsubsection{Risk Score}
\label{sec:risk}
To compute $S_{Risk}$, we first computed the \textbf{\ac{resonate} score} using the \ac{btd} with the hazard of ``roadway obstruction" shown in \cref{fig:btd}. To compute the collision rate $\lambda$, we analyzed the conditional relationships of \ac{btd}'s barriers and threats using the calibration set. The probability function of barriers $B1$ and $B2$ are dependent on the continuous-valued output of the \ac{ood} detector and the binary state of the anomaly detectors, which is captured using the following equation.

% . These relationships are captured using the following equation.

%  For this, we used the calibration set with normal scenes and scenes with different weather conditions and sensor failures, as discussed earlier.


\small
\begin{gather}
f_b(x=(B_1,B_2),s) = (1-P(x|s.m.LEC)) * \prod_{d\epsilon S^{B2}}{\frac{P(x|d)}{0.4} * f_{s}} \nonumber \\
P(x|s.m.LEC) = (1+e^{-0.049*(t.m.LEC-5.754)})^{-1}
\label{eqn:conditional_prob}
\end{gather}
\normalsize

Where, $P(x|s.m.LEC)$ is a sigmoid function used to capture the continuous values of the \ac{ood} detector, the discrete-valued probability of the anomaly detectors that constitutes the state-variables in $S^{B2}$. In our example, $B1$ and $B2$ were affected by the image quality, which we detect using the blur and occlusion detectors whose probabilities are reported in~\cref{fig:btd}. Also, $f_{s}$ is the failure rate of the sensors, which is assumed to be constant for both the camera and the radar sensors on which the barriers are dependent. Further, the probability function of $B3$ is conditionally dependent on the precipitation levels and the operation of the radar as shown in \cref{fig:btd}. These conditional relationships were inferred by clustering the calibration scenes based on the precipitation levels. In a similar approach, we also estimated the frequency of threat occurrence. In this example, the frequency of threats $T1$ and $T2$ was dependent on the road segments. That is, an intersection had a higher frequency of threats as compared to a side road. This information was aggregated from the calibration data and stored in a \ac{lut}. Finally, we used these probabilities to compute the dynamic collision rates and the system's dynamic risk (\ac{resonate} score) as discussed in \cref{sec:scoring}.  

Next, we computed the \textbf{Infraction score} from the simulator statistics $IS = 0.7 \cdot I_S + 0.8 \cdot I_R + I_{RD}$. Where $I_S$ is a stop sign infraction, $I_R$ is a red-light infraction, and $I_{RD}$ is the deviation in the route taken by the \ac{av}. These weights are chosen from the CARLA challenge setup~\cite{carla-challenge}. This score was added to the \ac{resonate} score to compute the $S_{Risk}$. Finally, we computed the risk threshold $\delta$ to be $0.65$, as discussed in \cref{sec:scoring}. 

\subsection{Baselines and Comparison Metrics} We compare our sampler to state-of-the-art baselines. \textbf{1) Random Search} is a technique that samples the scene variables uniformly at random from their respective distributions. \textbf{2) Grid Search} is a technique that exhaustively samples all the combinations of the scene variables in a given grid. \textbf{3) Halton Sequence Search}~\cite{halton1960efficiency} is a pseudo-random technique that samples the scene variables using co-prime as its bases. We compare these baselines using the following metrics, which align with the sampler objectives discussed in \cref{sec:ps}. 

\textbf{1) Total Risk Scenes (TRS)}: The proportion of the high-risk scenes sampled to the total scenes sampled ($N$).
\begin{equation}
\label{eqn:rsp}
\small
    TRS (\%) = \frac{1}{N}\sum_{i=1}^{N} s_i \quad \textnormal{if} \quad S_{Risk}^i > \delta
\end{equation}
Where $S_{Risk}^i$ is the risk across the $i^{th}$ sampled scene, and $\delta$ is the risk threshold computed across the calibration set. 

% $N$ is the total number of scenes sampled,

% \textit{2) Diversity ($D$)} is a measure widely used to evaluate the tradeoff between exploration and exploitation~\cite{jerebic2021novel}. We measure diversity using the number of clusters and the quality of the cluster population as shown in \cref{eqn:diverse}. The cluster quality is measured as the average $S_{Risk}$ of the cluster population.

\textbf{2) Diversity ($D$)}: We measure the coverage diversity using two cluster-based quantities. (1) the number of optimal clusters that can be generated from the $N$ sampled scenes, as measured using silhouette score~\cite{rousseeuw1987silhouettes}. (2) the variance of risk across each scene across all the cluster. These quantities are combined into computing the diversity score as follows. 

% cluster quality is measured as the variance across the average $S_{Risk}$ of the different clusters.
\begin{equation}
\small
\label{eqn:diverse}
    % Diversity = \sum_{i=1}^{T_C} \left(\frac{1}{P^i}\sum_{j=1}^{P^i} S_{Risk} \right)
    Diversity = \sigma^2\{\frac{1}{len(\mathcal{C})}(\sum_{i=1}^{len(\mathcal{C})} S_{Risk}^i)|\forall \mathcal{C} \in N\}
\end{equation}    
    % \sigma^2\{\left(\frac{1}{P^i}\sum_{j=1}^{P^i} S_{Risk} \right) \quad | \quad \forall i \in \mathcal{C}\}   

Where $\mathcal{C}$ is a cluster of scenes generated on the scene variables. $S_{Risk}^i$ is the risk of the $i^{th}$ scene in a cluster. To select the optimal number of clusters, we perform kmeans clustering~\cite{wagstaff2001constrained} using silhouette score as the selection metric.


% To cluster the scenes, we perform kmeans clustering~\cite{wagstaff2001constrained} on the scene variables. We then use the silhouette score~\cite{rousseeuw1987silhouettes} as the metric to select the optimal number of clusters. 

% That is, we choose the number of clusters that had the highest silhouette score.

\textbf{3) Search Time}: The overall time taken by the sampler to sample $N$ scenes and execute them in the simulator.


\subsection{Results}
\label{sec:results}
% To demonstrate our approach, we tasked the \ac{av} navigate different simulation scenes generated by the samplers. During these scenes, the \ac{ood} detector measures the martingale score, and the risk estimator estimates the collision rate $\lambda$ once every inference cycle. In these experiments, the simulation operates at a fixed rate of $20$ Frame Per Seconds. Also, to compare our samplers against the baselines, we executed each sampler for $250$ iterations. We started the samplers at the same initial condition with time-of-day = $45$ (noon) and a value of zero for the other variables. Also, instead of starting the \ac{gbo} sampler from scratch, we use the results from the random sampler to provide it a ``warm start". Further, for controlling the exploration vs. exploitation tradeoff, we empirically selected the following parameters. (1) Number of neighbors $K$ = 6, and neighborhood threshold $\tau$ = 10 for the \ac{rns} sampler, and (2) $\beta$ = 30 for the \ac{ucb} function of the \ac{gbo} sampler. 

% To demonstrate our approach, we tasked the \ac{av} navigate different simulation scenes generated by the samplers. During these scenes, the \ac{ood} detector measures the martingale score, and the risk estimator estimates the collision rate $\lambda$ once every inference cycle. In these experiments, the simulation operates at a fixed rate of $20$ Frame Per Seconds.

To compare our samplers against the baselines, we executed each sampler for $250$ iterations. We started the samplers at the same initial condition with time-of-day = $45^{\circ}$ (noon) and a value of zero for the other variables. Also, instead of starting the \ac{gbo} sampler from scratch, we provide it a ``warm start" using the results from the random sampler. Further, we empirically selected the following parameters for controlling the exploration vs. exploitation tradeoff. (1) Number of neighbors $K$ = 6, and threshold $\tau$ = 10 for the \ac{rns} sampler, and (2) $\beta$ = 30 for the \ac{ucb} function of the \ac{gbo} sampler. In these experiments, the simulation operates at a fixed rate of $20$ Frame Per Seconds. \cref{fig:sampler_3d} shows the qualitative comparison of the scenes sampled by the samplers. The random and Halton samplers explore the search space, but they cannot exploit it because of their passive search strategy. On the other hand, the grid sampler orderly exploits every point in the grid, which limits its exploration. In comparison, the \ac{rns} and \ac{gbo} samplers performs balanced exploration and exploitation. This is evident from the dense scene clusters at different regions of the search space. Further, we compared the samplers using the comparison metrics. 

\input{results/comparison-table2}

\input{results/infractions}

% Further, we also compared the samplers using the comparison metrics.  


\textbf{Total Risk Scenes}: \cref{Table:comparison} lists the total risk scenes generated by different samplers. As seen, the random, Halton, and grid samplers sampled $66$\%, $71$\%, and $56$\% of high-risk scenes, respectively. In comparison, the \ac{rns} sampler sampled 83\% and \ac{gbo} sampled 92\% high-risk scenes among the $250$ scenes that were sampled. Also, \cref{fig:infractions} illustrates the number of \ac{ood} scenes and scenes with infractions that were generated by the samplers in $250$ iterations. As seen, the \ac{gbo} and the \ac{rns} samplers generated higher \ac{ood} scenes compared to the baselines. Also, the \ac{rns} sampler sampled the highest scenes with infractions followed by \ac{gbo} and Halton samplers. The actual infractions are low even when the risk is high because. (1) the \ac{lec} controller was sufficiently trained (retraining the \ac{lec}, further reduced the infractions (See \cref{sec:discussion})), (2) the \ac{aebs} worked sufficiently well to stop the \ac{av}.


\input{results/initial-conditions}

% varying the time-of-day (T), precipitation (P), and cloudiness (C)

We also started the simulator at $5$ different initial conditions. (1) T = $0^{\circ}$ (dawn), (2) T = $45^{\circ}$ (noon), (3) T = $90^{\circ}$ (dusk), (4) T = $45^{\circ}$ (noon), P = 50\%, C = 50\%, and (5) T = $45^{\circ}$, P = 0\%, C = 50\%, and the other variables were set to zero. Each sampler was executed for $50$ iterations from these initial conditions. \cref{fig:initial} shows the high-risk scenes generated by the different samplers. The \ac{rns} and \ac{gbo} samplers generated high-risk scenes across the different starts as compared to the baselines. Among the baselines, the grid search generated higher high-risk scenes than the other two samplers. To note, different stating conditions did not affect the Halton sampler.

\textbf{Diversity}: To compute diversity, we 
extract the clusters by applying kmeans clustering analysis along with silhouette score. As seen in \cref{Table:comparison}, the scenes generated by the \ac{rns} and \ac{gbo} samplers could be clustered into $6$ and $4$ clusters. Whereas the scenes generated by the Halton, grid, and random samplers could only be clustered in $2$, $2$, and $3$ clusters, respectively. We used these clusters to compute the diversity score in \cref{eqn:diverse}. As seen, the \ac{gbo} and \ac{rns} samplers had a higher diversity score of $0.63$ and $0.19$ as compared to the Halton, random, and grid samplers, which had scores of $0.07$, $0.02$, and $0.13$, respectively. The \ac{gbo} and \ac{rns} samplers had higher coverage diversity because they sampled higher scene clusters from risky regions of the search space.


% despite having a lower number of clusters than the \ac{rns} sampler. This is because \ac{gbo} sampled clusters belonged to regions of the search space that had higher $S_{Risk}$. This is evident from \cref{fig:cluster}, which reports the cluster wise $S_{Risk}$ of all the samplers. In comparison, the baselines had a lower diversity score. 

% For this, we computed the variance across the average $S_{Risk}$ of the different clusters.

% It can be seen that the other samplers missed the critical high-risk areas that the \ac{gbo} sampler could identify. 

\begin{figure}[!t]
\input{results/cluster}
 \vspace{-0.1cm} 
 \input{results/cluster1}
\footnotesize
\centering
\setlength{\abovecaptionskip}{2pt}
\caption{The variance of $S_{Risk}$ across scene clusters generated by different samplers. Our samplers generate more clusters with a high variance of $S_{Risk}$. Y-axis shows the number of clusters, and the Y-axis shows the $S_{Risk}$ score.}
\label{fig:cluster}
\vspace{-0.1in}
\end{figure}

% \input{results/samples}

\textbf{Search Times}: We report the search times of the samplers in \cref{Table:comparison}. The random, Halton, grid, and \ac{rns} samplers have comparable search times of $323$, $315$, $309$, and $332$ minutes, respectively. However, the \ac{gbo} sampler required the highest search time of $897$ minutes because of its scalability issue discussed in \cref{sec:gbo_sampler}. Further, for a direct comparison, we counted the number of scenes sampled by each sampler within a fixed budget of $60$ minutes. The random, Halton, grid and 
\ac{rns} samplers sampled $47$, $51$, $49$, and $46$ scenes in $60$ minutes. But, the \ac{gbo} sampler only sampled $19$ scenes. 

% in the allotted time. 



% The \ac{gbo} sampler suffers from the scalability issue discussed earlier. This causes the \ac{gbo} sampler to sample only $19$ scenes, while all the other samplers roughly sample $40$ scenes in the allotted time. 

\subsection{Discussion}
\label{sec:discussion}
The key takeaways from the experiments are. \underline{First}, we observe that the \ac{rns} and \ac{gbo} samplers outperform the baselines by generating a higher percentage of high-risk scenes (first objective). \underline{Second}, we observe that the scene generated by the \ac{rns} and \ac{gbo} samplers could be clustered into more clusters with higher variance compared to the baselines (second objective). \underline{Third}, the \ac{gbo} sampler is the most effective in generating high-risk scenes, and its informed exploration results in diverse search. But, the use of \ac{gp} model increases the search time. In comparison, the \ac{rns} sampler is efficient and requires lower search times to generate high-risk scenes. 

% A few of these scenes were used in training $M_{retrain}$.


\underline{Lastly}, the high-risk scenes identified by our samplers can be used to improve the system's \acp{lec}. To illustrate, the \ac{av} system in our case study was susceptible to scenes from the evening with high precipitation ($T<50$ and $P<50$) as identified by our samplers. So, we trained a new \ac{lec} controller model $M_{retrain}$ on a dataset that contained both the original train scenes and $50$ high-risk scenes sampled by the \ac{rns} sampler. We trained the model for $50$ epochs and saved several model weights, and utilized the weights that optimized the \ac{av}'s driving proficiency. We then compared the performance of the original model $M_{orig}$ (model trained on original training scenes) and the retrained model $M_{retrain}$ in terms of the actual system infractions, which included collision, running a red light or stop sign, and route deviation. The comparison is shown in \cref{fig:retrain}, and for this, we curated $80$ operational scenes that included random scenes and scenes where the system previously failed. We observed that $M_{retrain}$ had only $6$ scenes with infractions as compared to $11$ scenes of $M_{orig}$. That is, retraining the model on the high-risk scenes reduced the system infractions, especially in the scenes from the highlighted region where it previously had higher infractions. Additionally, we observed that $M_{retrain}$ had improved driving proficiency with fewer route deviations for the high-risk scenes. But in general, both the models performed several red light infractions, and retraining did not address the problem.



% This is because the perception \ac{lec} does not learn to effectively brake on encountering a red signal. 

\begin{figure}[t]
\centering
 \includegraphics[width=\columnwidth]{figures/retrain.pdf}
\caption{Performance of $M_{retrain}$ and $M_{orig}$ models. $M_{retrain}$ model had fewer infractions, especially in the scenes from the region highlighted.}
\label{fig:retrain}
\vspace{-0.1in}
\end{figure}




% our samplers can be used to identify the operating conditions in which the system is susceptible to failure. The data from these conditions 


% . This is because these scenes were identified to be high-risk by the sampler and, they were used to train the new model.   





% history of the search space is available. (b) there is no time budget for the search. However, the \ac{rns} sampler is efficient with lower search times compared to the \ac{gbo} sampler. 


% and it can be used when (a) some history of the search space is available. (b) there is no time budget for the search process. However, when no past search information is available, the \ac{rns} sampler can be used.  









==> Accepted/individual-sections/problem-statement.tex <==
\section{Problem Formulation}
\label{sec:ps}
\subsection
We use an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to set up the problem. The \ac{av} is tasked to navigate an urban town with complex traffic scenarios including changing weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. The \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation. Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.

% Given this simulator, the \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation.  

The \ac{lec} is trained on a training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes. A scene $s$ is a short time-series trajectory (typically 30 seconds to 60 seconds) of the \ac{av}'s journey in the environment. It can be represented as a sequence of entries at each time step, where each entry is defined by different environmental variables ($e_v$) and agent variables $a_v$. The environment can be captured using different structural variables (e.g., road segments, waypoints, road geometry) and temporal variables (e.g., weather, time-of-day, traffic). The agent variables can be operating modes, sensor faults, failure modes, etc. These scene variables $s_v$ are mostly defined by a distribution $\mathcal{P} \in [lower,upper]$. The combination of these scene variables form a search space $\mathcal{D}$, which can be sampled to generate different scenes. However, each of these variables may have different constraints $C$ as discussed earlier. 
For example, in the CARLA case study, the CARLA map defines the list of adjacent road segments, which forms the structural constraints. Similarly, there may be constraints on the rate of change in the values of the environmental variables. For example, the precipitation levels cannot drastically change from 10\% to 90\%, it can only gradually increase at a defined rate. Also, each scene is associated with a risk score $R_S$ estimated by the risk estimator. 


Given this setup, the problem we study in this work is to design sampling approaches that can find the following.  

\begin{enumerate}
    \item Given the scene variables $s_v$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate a scene $s_i$ that has a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
    
    \item Given the scene variables $s_v$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate cluster of similar scenes $C_s$ that have a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
\end{enumerate}
    

% \begin{problem}
% \label{prob:high-risk scene}
% Given the scene variables $S_V$ and the search space $\mathcal{D}$, generate a scene $s_i$ that has a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
% \end{problem}

% \begin{problem}
% \label{prob:cluster scene}
% Given the scene variables $S_V$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate cluster of similar scenes $C_s$  that have a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
% \end{problem}


% With this set up, we can define the problems we study as follows:

% \ac{lec} is trained on sensor data in the training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes.

==> Accepted/individual-sections/problem-statement1.tex <==
\section{Problem Formulation}
\label{sec:ps}
We consider the autonomous \ac{cps} to be operating in an environment, characterized by two sets of variables $\mathbb{E}: x \rightarrow \Re^{+}$ and $\mathbb{S}: y \rightarrow \Re^{+} \times \Re^{+}$. The $\mathbb{E}$ are the environmental variables like rain, traffic density, time-of-the-day. The $\mathbb{S}$ are structural variables related to roadway features and are characterized by waypoints $w$ denoted by a two-dimensional matrix of latitude and longitude. Also, each waypoint can be mapped to a road segment. In addition, we consider the set of faults in the system sensors and actuators $F: x \rightarrow {0,1}$. For a particular operating environment, there can be several environment variables $e \in \mathbb{E}$, several possible waypoints $w \in \mathbb{S}$, and several sensors in the system that can fail $f \in \mathbb{F}$. The \ac{cps} is trained through a collection of scenes $\mathcal{T}$, where each scene $s$ is an ordered sequence of $K$ sampled observations $< s_i=(\mathbb{E}_i, \mathbb{S}_i, \mathbb{F}_i) >_{i=1}^{K}$. We collectively refer to these variables as the scene variables $s_V$. Given each scene $s_i$, we can associate the likelihood of hazard rate ($\lambda$) for every hazard that is identified for the system. The system can have a collection of hazards $\{H_1,H_2,\cdots,H_n\}$ stemming from its components (e.g., software, hardware) or its operating conditions. Each identified hazard will have an associated hazard rate estimated using the dynamic assurance routines ($DA: s \rightarrow \lambda$) introduced in \cref{sec:risk_estimation}. The hazard rate can be used to compute the likelihood of the hazard occurrence ($1-e^{-\lambda \cdot t}$) in each time unit $t$. The estimated likelihood of hazard for different hazard conditions put together constitutes the system's operational risk $S_{Risk}$. 

 
% and provides the features of the road: gradient, elevation, number of lanes.

\input{results/constraints}

\begin{figure*}[!ht]
\centering
 \includegraphics[width=0.9\textwidth]{figures/workflow10.pdf}
 \caption{Overview of the proposed approach, which includes a \acl{sdl} integrated with two samplers and a scoring function for generating high-risk scenes. The samplers perform active sampling using the feedback loop (red dotted line). Our approach is designed for the testing phase of \ac{cps}.}
 \label{fig:workflow}
% \vspace{-0.1in}
\end{figure*}


% \footnote{It is common to use latitude and longitude as the waypoint}.

Also, given a sequence of samples in the scenes, physical constraints govern the temporal evolution of the sampled values. For example, a constraint on an environmental variable $e \in \mathbb{E}$ governs that $|s_i^e-s_{i+1}^e| \leq \alpha_e \in \Re^+$. Similarly, the waypoints across a scene are governed by routability property. To explain this, we use the sampling constraints $\mathcal{SC}$ (See \cref{Table:constraints}) that we applied for an \ac{av} case study that will be discussed in \cref{sec:casestudy}. The road segment is governed by the constraint that the distance between two selected waypoints cannot be greater than $10$ meters. This constraint regulates that the road segment is orderly selected. The environmental variables have constraints on how much their values change between consecutive scenes. The traffic density has constraints on its value and is also dependent on the type of road segment (e.g., crossroads, intersections). Also, we did not place any constraints on the fault variables. Now, given this setup, we want to address the following problem. 

% Without these constraints, we found the sampled scene sequence was unrealistic. Two such scenes were  

% the trained \ac{cps} and its operating conditions, we want to address the following problems. 

\begin{problem}
\label{prob:high-risk scene}
Given a threshold $\delta$ (computed across the calibration set of scenes), sample $N$ scenes that maximizes the risk $\max(sum(S_{Risk} - \delta))$. In addition we want to ensure that the scene variables are diverse. We call a scene with ($S_{Risk} - \delta) > 0$  as a high risk scene.

% diversity across the clusters is maximized 


% $\max(\sigma^2\{\frac{1}{len(\mathcal{C})}\sum_{i=1}^{len(\mathcal{C})} (S_{Risk}^i-\delta) |  \forall \mathcal{C} \in N\})$ 
\end{problem} %\textcolor{red}{This is not correct. The diversity is on the features of the scenes and should not have anything to do with the $S_{Risk}$. Perhaps just explain this is in simple words if you cannot explain in mathematics}


% maximizes the diversity $\max(\sigma^2(S_{Risk} - \delta))$. 

% dissimilarity of the $N$ Scenes that have been sampled.
%Find scenes that have $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from previously observed scenes. 


% \begin{problem}
% \label{prob:cluster scene}
% Find clusters of similar scenes that have $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from previously observed scenes 
% \end{problem}

% Where $\delta$ is the risk threshold computed across the previously observed train scenes. A scene with $S_{Risk} - \delta > 0$ is termed to as high-risk scene in this work. Now, our goal in this work is to design a ``\textit{Sampler}" which can address the problem. The problem can be expressed as two objectives of the sampler. The first objective of the sampler is to sample a higher number of high-risk scenes. The second objective of the sampler is to sample a higher number of scenes clusters, such that the variance of risk across the clusters is high. While the first objective measures the sampler's capability of finding the region of the search space with high-risk scenes, the second measures the sampler's diversity,which is a measure of the sampler's exploration vs. exploitation trade-off. High diversity is desirable to better cover the search space~\cite{jerebic2021novel}. We measure diversity in terms of a quantitative metric (measured using the number of the cluster) and a qualitative metric (measured using the variance of risk across clusters). 

% Recall, our goal is to design a %``\textit{Sampler}" which can address the problem. 
%The problem can be expressed as two objectives. The first objective is to sample a large number of high-risk scenes. The second objective is to ensure diversity across the sampled scenes. 
%higher number of scenes clusters, such that the variance of risk across the clusters is high.
While the first objective measures the sampler's capability of finding the region of the search space with high-risk scenes, the second measures the sampler's coverage diversity, which represents the sampler's capability to balance between exploration vs. exploitation. A sampler with high diversity is desirable for better coverage of the search space~\cite{jerebic2021novel}. We measure diversity in terms of a quantitative metric (measured using the number of the optimal clusters, as measured using silhouette score~\cite{rousseeuw1987silhouettes}) and a qualitative metric (measured using the variance of risk across each scene across all clusters). 




% First, sample a higher number of high-risk scenes. This measures the sampler's capability of finding the region of the search space with high-risk scenes. Second, sample a higher number of scenes in clusters, such that the variance of risk across the clusters is high. This measures the sampler's diversity, which is a measure of the sampler's exploration vs. exploitation trade-off. High diversity is desirable to better cover the search space~\cite{jerebic2021novel}. We measure diversity in terms of a quantitative metric (measured using the number of the cluster) and a qualitative metric (measured using the variance of risk across clusters). 




% Diversity is a measure used to evaluate the exploration vs. exploitation trade-off, which is a desirable property to better cover the search space~\cite{jerebic2021novel}. So, our objective is to maximize the diversity. 

 
% to have higher number of clusters and higher variance

% Second, sample scenes in clusters such that the variance of risk across the clusters is maximized. We use variance as the measure of the sampler's diversity. The diversity is a measure widely used to evaluate the exploration vs. exploitation trade-off~\cite{jerebic2021novel}. In our setup, it is measured as the variance of $S_{Risk}$ across the clusters that are generated from the $N$ sampled scenes. So, higher the variance, better is the exploration vs. exploitation strategy. 

% Now, our goal in this work is to design a ``\textit{Sampler}" which can address the problem. 
% Addressing the problem is relevant for the uses cases briefly introduced earlier. That is, addressing the first part of the problem will generate the high-risk scenes that can be used for testing and validating the system. Addressing the second part will generate clusters of similar high-risk scenes which can be used for continually improving models.  

% We refer to high-risk scenes when we use the term ($S_{Risk} - \delta$)

% To explain these problems, we setup an \ac{av} case study in CARLA simulator~\cite{dosovitskiy2017carla}. In this example, an \ac{av} is tasked to navigate an urban town with complex traffic conditions, adverse weather conditions (e.g., high lighting level, high precipitation), and sensor faults (e.g., camera failure). These simulation parameters are the scene variables, which we sample based on the sampling constraints in \cref{Table:constraints} to generate scenes with varying operating conditions. Also, to evaluate the \ac{av}'s performance, we leverage the infraction metrics returned by the CARLA autonomous driving challenge ~\cite{carla-challenge}. Specifically, we use the system infractions like running a red light, running a stop sign, route deviation, off-road driving, etc. Now, given this simulation setup, the goal of the \ac{av} is to navigate the different scenes without collisions. For this, the \ac{av} is augmented with safety components anomaly detectors, an \ac{ood} detector and a risk estimator~\cite{hartsell2021resonate} for dynamic assurance routines. These components together estimate the \ac{av}'s hazard rate and its operational risk in a given scene ($DA: S \rightarrow S_{Risk}$). With this setup, we train an \ac{lec} controller to operate the \ac{av} and calibrate the safety components with several train and calibration scenes which we will discuss in \cref{sec:evaluation}. Now, given the trained \ac{av}, our goal is to design a sampler for sampling high-risk test cases for the \ac{av}.

% find test scenes that are of high-risk to the \ac{av}. For this, our goal is to design a sampler that can address the two problems discussed above.


==> Accepted/individual-sections/problem-statement2.tex <==
\section{Problem Formulation}
\label{sec:ps}
\textbf{Problem Setup}: To set up the problem, consider an autonomous \ac{cps} operating in a simulator. This system uses an \ac{lec} for navigation, and it is augmented with safety components such as anomaly detector, \ac{ood} detector, and risk estimators for dynamic assurance and estimating the system's operational risk. These components are usually trained and calibrated on sensor data (e.g., camera images, radar signals) collected from a training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes. 

A scene $s$ is a short sequence of sampled observations. Each sample is an indexed entry from the scene and provides a value to three class of variables 

(typically 30 seconds to 60 seconds) of the system's journey in the environment. It can be represented as a time-stamped sequence of entries, where each entry is defined by different environmental variables ($e_v$) and agent variables $a_v$. The environment can be captured using different structural variables (e.g., road segments, waypoints, road geometry) and temporal variables (e.g., weather, time-of-day, traffic). The agent variables can be operating modes, sensor faults, failure modes, etc. These scene variables $s_v$ are mostly defined by a distribution $\mathcal{P} \in [lower,upper]$. 

The combination of these scene variables forms a search space $\mathcal{D}$, which can be sampled to generate different scenes. However, these variables may have constraints that need to be included during sampling. For example, the structural variables such as road segments and waypoints may have sequential ordering constraints defined by the simulator's map. Similarly, temporal variables like the weather parameters (e.g., lighting) may have constraints on the rate at which their values change. In addition, each scene is associated with a risk score $S_{Risk}$ estimated by the risk estimator. Now, given the trained system with the calibrated risk estimator, we want to generate scenes in which the system is susceptible to failure. For this, our goal is to design a sampler that can address the following problems.    

% in the CARLA case study, the CARLA map defines the list of adjacent road segments, which forms the structural constraints. Similarly, there may be constraints on the rate of change in the values of the environmental variables. For example, the precipitation levels cannot drastically change from 10\% to 90\%, it can only gradually increase at a defined rate. Also, each scene is associated with a risk score $S_{Risk}$ estimated by the risk estimator. Given this set up, the goal is to test the \ac{cps} across scenes where it fails. For this, the goal of this work is to design a sampler that can address the following problems.  
    
\begin{problem}[Sample High-Risk Scene]
\label{prob:high-risk scene}
Given the scene variables $S_V$, the search space $\mathcal{D}$, and the sampling constraints, sample scenes $s_i$ that have risk $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from the previously observed scenes. 
\end{problem}

\begin{problem}[Sample Cluster of High-Risk Scenes]
\label{prob:cluster scene}
Given the scene variables $S_V$, the search space $\mathcal{D}$, and the sampling constraints, sample clusters of similar scenes $C_s$ that have risk $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from the previously observed scenes 
\end{problem}

\textbf{Case Study}: We consider an \ac{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to explain these problems. In this example, an \ac{av} is tasked to navigate an urban town with complex traffic conditions, adverse weather conditions (e.g., high lighting level, high precipitation), and sensor faults (e.g., camera failure). These simulation parameters are the scene variables, which we sample to generate scenes with varying operating conditions. Also, to evaluate the \ac{av}'s performance, we leverage the infraction metrics returned by the CARLA autonomous driving challenge ~\cite{carla-challenge}. Specifically, we use the system infractions like running a red light, running a stop sign, route deviation, off-road driving, etc. Now, given this simulation setup, the goal of the \ac{av} is to navigate the different scenes without collisions. For this, the \ac{av} is augmented with several anomaly detectors, an \ac{ood} detector and a risk estimator~\cite{hartsell2021resonate} to estimate the \ac{av}'s risk of collision across an operating scene. The \ac{lec} controller is trained, and the risk estimator is calibrated using several train and calibration scenes. The specifics of the \ac{av} setup and training are discussed in \cref{sec:evaluation}. Now, given the trained \ac{av}, our goal is to find test scenes that are of high-risk to the \ac{av}. For this, our goal is to design a sampler that can address the two problems discussed above.




% Now, given the trained \ac{av}, we want to test it across different scenes where it is susceptible to failure. For this, our goal is to design a sampling approach that can sample. (1) scenes $s_i$ with different operating conditions and camera faults that has a risk greater than the risk across the training scenes. and (2) a cluster of scenes $C_s$ with similar operating conditions and camera faults that have a risk greater than the risk across the training scenes. 

% To address these problems, we design two sequential sampling approaches that considers the sampling constraints and provides an explicit control over the exploration and exploitation of the search space. The sampling approaches are discussed in the following section. 

% To explain these problems, we consider an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla}. We rely on the CARLA autonomous driving challenge ~\cite{carla-challenge} setup that allows simulating complex traffic scenes and it also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. This set up allows us to generate different traffic scenes by varying weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. In addition, it also allows us to inject different faults (e.g., camera occlusion, camera blur) into the \ac{av}'s sensors.  

% The \ac{av} in this set up is driven by a navigation \ac{lec} controller and it has an \ac{ood} detector and a \ac{resonate} risk estimator~\cite{hartsell2021resonate} as the safety components for runtime monitoring. The controller and the components are trained and calibrated using a set of scenes $\mathcal{T}$ generated by randomly varying the weather, traffic and pedestrian density, and road segments. Each of these scenes has an associated risk $R$ of \ac{av}'s collision as estimated by the risk estimator. Now, given simulator set up and the \ac{av}, the goal is to design a sampler that can find. (1) a single scene $s_i$ with different operating conditions and camera faults that has a risk greater than the risk across the training scenes, and (2) a cluster of scenes $C_s$ with similar operating conditions and camera faults that has a risk greater than the risk across the training scenes.     


% Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.

% \subsection{Case Study}
% We use an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to set up the problem. The \ac{av} is tasked to navigate an urban town with complex traffic scenarios including changing weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. The \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation. Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.



==> Accepted/individual-sections/related-works.tex <==
\section{Related Work}
\label{sec:rw}
Tools like Dakota~\cite{dalbey2021dakota} with sampling approaches like incremental sampling, importance sampling, and adaptive sampling have been long available for uncertainty quantification in engineering design. Such samplers have recently gained interest for sampling simulation-based scenes in the \ac{av} domain. Several domain-specific \acp{sdl} like Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} have been designed for specifying scenarios of complex traffic conditions and operating conditions to identify counterexamples that affect the system's safety. These languages are mostly designed for the \ac{av} domain to work with the CARLA simulator~\cite{dosovitskiy2017carla}. Also, they use probabilistic samplers that sample scenes across the entire search space formed by the combination of scene variables. For example, Grid search is a popular passive sampler, which takes a single risky scene as the starting condition and generates similar risky scenes around it. However, manual tuning makes the grid sampler labor-intensive and time consuming. For accelerating the search process, an alternate approach~\cite{zhao2017accelerated} uses importance sampling to identify important scene variables and sample scenes using them. Worst-Case Scenario Evaluation~\cite{ma1999worst} is another approach that uses model-based optimization to identify the weakness of the system and uses this information to generate worst-case disturbances. VERIFAI~\cite{dreossi2019verifai} software toolkit has several passive samplers like random search, Halton search~\cite{halton1960efficiency}, and active samplers like cross-entropy optimization and \acl{bo}. But, these samplers cannot control the exploration vs. exploitation trade-off during sampling. This is addressed by a multi-armed bandit sampler that balances the two strategies~\cite{viswanadha2021parallel}. 


Also, recently, there has been growing interest in using generative models for generating risky scenes~\cite{ding2018new,vardhan2021rare,o2018scalable,ding2020learning}. In this approach, scenes are randomly sampled from a distribution learned by a generative model instead of sampling from the entire search space (as performed by the samplers discussed above). For example, Ding, Wenhao, \emph{et al.}~\cite{ding2020learning} use an autoregressive model to factorize the scene variables into conditional probability distributions, which are then sampled to generate risky traffic scenes. In a prior work~\cite{ding2018new}, they have also used a \acl{vae} to project high-dimensional traffic information into a lower-dimensional latent space, which is sampled to generate critical traffic scenes. Vardhan \emph{et al.}~\cite{vardhan2021rare} use a Gaussian Mixture Model to find the corner case scenes in the training set that is not well learned by the system. Another approach~\cite{o2018scalable} uses generative adversarial imitation learning to perform adaptive importance-sampling to learn rare events from an underlying data distribution. 



% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 

% The generation of scenes covering the entire range of expected environmental conditions has become an important study for testing and validating autonomous \ac{cps}. Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} are well-known domain-specific \acp{sdl} used for scene generation. These languages have been equipped with probabilistic samplers to sample different values for the scene variables. Grid search is a brute force approach widely adopted in the industry. In this approach, a previously identified risky scene is used as the initial condition, and the grid around it is searched to sample risky scenes~\cite{ding2020learning}. This approach requires prior information of the risk scenes and can be labor-intensive. Instead of starting from manually identified risk scenes, an importance sampling approach for accelerated identification of high-risk scenes is proposed ~\cite{ding2020learning}. VERIFAI~\cite{dreossi2019verifai} provides several sampling approaches like random search, Halton search, cross-entropy optimization, and \acl{bo}, which is integrated with Scenic~\cite{fremont2019scenic} to generate scenes with counterexamples. Also, recently, the scene sampling process is formulated as a multi-armed bandit problem, which seeks to balance between exploration vs. exploitation ~\cite{viswanadha2021parallel,viswanadha2021addressing}.

% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 

==> Accepted/individual-sections/rw.tex <==
\section{Related Work}
\label{sec:rw}
% The task of generating high-risk or safety critical scenes has been addressed in the literature using. 1) sampling-based approaches, 2) 

% can be broadly classified into three categories. 1) sampling

% The generation of high-risk or safety-critical scenes in simulation has gained significant interest in recent years. 
Tools like Dakota~\cite{dalbey2021dakota} with sampling approaches like incremental sampling, importance sampling, and adaptive sampling have been long available for uncertainty quantification in engineering design. Such samplers have recently gained interest for sampling simulation-based scenes in the \ac{av} domain. Several domain-specific \acp{sdl} like Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} have been designed for specifying scenarios of complex traffic conditions and operating conditions to identify edge cases and counterexamples that affect the system's safety. These languages are mostly designed for the \ac{av} domain to work with the CARLA simulator~\cite{dosovitskiy2017carla}. These languages are equipped with probabilistic samplers to sample values for scene variables from their distribution ranges, thus generating different scenes. For example, the Scenic language is integrated with the VERIFAI~\cite{dreossi2019verifai} software toolkit that has several passive samplers like random search, Halton search~\cite{halton1960efficiency}, and simulated annealing, which do not use the previous results to perform an informed sampling. Additionally, they include active samplers like cross-entropy optimization and \acl{bo}, which use a feedback loop of previous results in the sampling process. These samplers cannot control the exploration vs. exploitation tradeoff during sampling. To address this, a multi-armed bandit sampler that balances the two strategies is proposed~\cite{viswanadha2021parallel}. 

% As discussed by Ding, Wenhao, \emph{et al.}~\cite{ding2020learning}, g

There have also been other approaches. Grid search is a popular passive sampling approach used in industry. Here, a previously identified risky scene is used as the initial condition, and the grid around is searched to sample similar risky scenes. Manual tuning makes the grid sampler labor-intensive and time consuming. For accelerating the search process, an alternate approach~\cite{zhao2017accelerated} uses importance sampling to identify important scene variables and sample scenes using them. Worst-Case Scenario Evaluation~\cite{ma1999worst} is another approach that uses model-based optimization to identify the weakness of the system and uses this information to generate worst-case disturbances. 

In addition to the conventional samplers, there have recently been growing interests in using deep generative models for generating risky scenes~\cite{ding2018new,vardhan2021rare,o2018scalable,ding2020learning}. These approaches sample scenes from a learned distribution instead of sampling from the entire search space. Ding, Wenhao,\emph{et al.}~\cite{ding2020learning} use an autoregressive model to factorize the scene variables into conditional probability distributions, which are then sampled based on conditional dependence to generate risky traffic scenes. In a prior work~\cite{ding2018new}, they have also used a \acl{vae} to project high-dimensional traffic information into a lower-dimensional latent space, which is sampled to generate critical traffic scenes. Vardhan \emph{et al.}~\cite{vardhan2021rare} use a Gaussian Mixture Model to find the corner case scenes in the training set that is not well learned by the system. Another approach~\cite{o2018scalable} uses an ensemble of generative adversarial imitation learning to perform adaptive importance-sampling to learn rare events from an underlying data distribution. 



% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 















% The generation of scenes covering the entire range of expected environmental conditions has become an important study for testing and validating autonomous \ac{cps}. Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} are well-known domain-specific \acp{sdl} used for scene generation. These languages have been equipped with probabilistic samplers to sample different values for the scene variables. Grid search is a brute force approach widely adopted in the industry. In this approach, a previously identified risky scene is used as the initial condition, and the grid around it is searched to sample risky scenes~\cite{ding2020learning}. This approach requires prior information of the risk scenes and can be labor-intensive. Instead of starting from manually identified risk scenes, an importance sampling approach for accelerated identification of high-risk scenes is proposed ~\cite{ding2020learning}. VERIFAI~\cite{dreossi2019verifai} provides several sampling approaches like random search, Halton search, cross-entropy optimization, and \acl{bo}, which is integrated with Scenic~\cite{fremont2019scenic} to generate scenes with counterexamples. Also, recently, the scene sampling process is formulated as a multi-armed bandit problem, which seeks to balance between exploration vs. exploitation ~\cite{viswanadha2021parallel,viswanadha2021addressing}.

% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 

==> Accepted/old-text/paper.tex <==
\section{Introduction}
\acp{cps} with autonomous capabilities are being actively deployed to operate in several safety-critical domains such as automotive, military, medical, etc. Especially in the automotive domain, \acp{av} have emerged to operate in the air, ground, and underwater. These systems mostly use \acp{lec}, which are machine learning (popularly deep learning) models to perform tasks such as navigation planning or predict control actions such as steer and speed. These components are mostly trained on sensor data that is aggregated from a training scenario. A scenario is a distribution over several scenes. A scene is a short time series of similar operating conditions contextualized by several spatial (e.g., road segment type, segment length) and temporal (e.g., weather, time-of-day, traffic density) parameters. They are then tested against a testing scenario that may have scenes which are similar or differ from the set of scenes in the training scenario. \acp{lec} have shown impressive performance for automotive driving tasks \cite{bojarski2016end} when the test scenes are similar to the training scenes. However, they have shown to be susceptible \cite{pei2017deepxplore,tian2018deeptest} to test scenes that are rare (e.g., accidents, tunnels, snow, fog) to occur. These rare events can increase the system's likelihood of a consequence as determined in our previous work \cite{hartsell2021resonate}. So, it is required to gather data and retrain these components on these scenes with rare events to prevent them from getting into a consequence. However, collecting real-world data of rare events is either expensive, time-consuming, or in most cases not feasible. 

% A popular example for this is the NVIDIA DAVE-II \ac{cnn} model ~\cite{bojarski2016end} that consumed a stream of forward facing camera images to predict the steering control for the car. Despite their exceptional performance, these models have shown to be susceptible \cite{pei2017deepxplore,tian2018deeptest} to corner case scenes that are rare (e.g., accidents, tunnels, snow, fog) to occur. These rare events can increase the system's likelihood of a consequence as determined in our previous work \cite{hartsell2021resonate}. So, it is required to gather data and retrain the models from these rare event scenarios to prevent them from getting into a consequence. However, collecting real-world data of rare events is either expensive, time-consuming or in most cases not feasible.

Recently, there has been a growing interest in using simulators like CARLA \cite{dosovitskiy2017carla} and gazebo \cite{koenig2004design} to recreate rare events that are not possible in real world. Then, the data generated from these scenarios are used to train and test the models. However, generating meaningful scenarios that are realistic can be a non-trivial task because of the large parameter state space from which the scenes have to be selected  ~\cite{fremont2019scenic}. To explain, let us consider that we want to generate data from a scenario of scenes with varying the weather parameters such as cloud, precipitation and precipitation levels. Suppose we uniformly at random sampled these parameter distributions over there ranges, then: (1) we could get a sample combination that is not realistically possible in real-world. For example, we could get cloud = 0\%, precipitation = 100\%, and precipitation level = 0\%, which is not realistic. Data from such unrealistic scenarios may not be useful for training the system, (2) we could miss sample combinations that could be realistic and happen in real-world. For example, we could miss generating cloud = 100\%, precipitation = 100\%, and precipitation level =10 0\%, which is a realistic and critical scene that could lead the system into a consequence, and (3) randomly sampling the entire state space   

To generate meaningful and realistic scenes, several domain-specific \acp{sdl} like Scenic \cite{fremont2019scenic} and MSDL \cite{msdl} with probabilistic sampling capabilities are available. These languages provide a language syntax to describe scene parameters like weather, traffic density, vehicle position, along with a probabilistic sampling capability to selectively sample the values for the scene parameters over a distribution. Also, instead of randomly sampling the parameters, these languages provide a closed loop sampling mechanism that problematically samples the values for the parameters that maximizes or minimizes an objective function. These functions are metrics like time-to-collision, distance-to-collision, collision history, etc. Although, these metrics are safety related, they are mostly one-dimensional and do not cover all the aspects related to the safety of the system.  

In this paper, we present a risk-aware scenario generation mechanism for autonomous \acp{cps}. The goal of our mechanism is to start from an initial driving scenario and then search for scenes that could result in a system consequence. To achieve this, we provide a scenario generation workflow that includes a simple \acl{sdl} that describes the parameters of a scene and their distribution ranges, a pluggable sampling engine with several samplers like random search, bayesian optimization and reinforcement learning, and a set of sampling rules that govern how the scenes can be composed. To facilitate the sampler, we use a novel risk-based metric as the objective function to maximize. For this we use the \ac{resonate} framework ~\cite{hartsell2021resonate} that was introduced in our previous work. The framework uses the design-time conditional probabilities computed from a \ac{btd} along with runtime state of the system (e.g., anomaly detectors, fault diagnosis) and environment information (e.g., weather conditions) to compute the dynamic risk of a system consequence as it operates. Furthermore, we keep updating the \acp{btd} conditional probabilities and the risk scores in \ac{resonate} as the system explores new and rare event scenes. We implement our mechanism for an \ac{av} example in the CARLA simulator \cite{dosovitskiy2017carla} and through comprehensive simulations across 1000 executions, we show that the system identifies the scenes leading to system consequence and updates the risk.


% Recently, there is a growing interest in assessing the dynamic risk of the autonomous \ac{cps}, which is a metric that uses the information about the state of the system and the environment to assess the safety of the system. For example, in our previous work ~\cite{hartsell2021resonate}, we introduced the \ac{resonate} framework that used the design-time conditional probabilities computed from a \ac{btd} along with runtime state of the system (e.g., anomaly detectors, fault diagnosis) and environment information (e.g., weather conditions) to compute the dynamic risk of a collision for the system. Since, the risk score covers system information from a wide variety of sources, we will use it as the objective function in the samplers introduced in this work.   





% These models are trained using sensor data that is collected from several scenes that are gathered during design time. A scene is short time series of similar images contextualized by certain environmental features such as weather, brightness, road conditions, traffic density, among others, as shown in \cref{fig:image-features}. These features are referred to as semantic labels \cite{nuimage} or generative factors ~\cite{higgins2016beta}, and in this paper, we refer to them as features. These features can take continuous or discrete values, and these values can be sampled for generating different scenes as shown in \cref{fig:image-features}. The images from these scenes are collectively used for training the \ac{dnn}. These features effectively specify the context in which the system is operating and influence the sensitivity and correctness of the \ac{dnn}'s predictions, especially in cases where the features representing the scenes used for training do not cover all the values found in real-world. In this work, we primarily focus on perception \acp{dnn}, so we define the problem in terms of images.

% Abhishek Points: 

% \begin{itemize}
%     \item Given an initial scene, identify next N scenes that maximize the probability of an event (e.g., collision)
    
%     \item Definition of a scene is on environment, sensor, other vehicles, and road topology 
    
%     \item Global rules : that describe the sampling rules: {each variable can taken certain value, temporal sequencing constraints} 
    
%     \item This paper is about building this language and defining the sampling engine that helps collect the data 
% \end{itemize}

% The proposed contributions of this work are:

% \begin{itemize}
%     \item We present a scene selection and generation mechanism that selects the scene parameters which maximizes the scene objective. In this case the objective function are the system consequences like collision, system's risk of collisions, etc. The scene parameters are used to run the simulation.
    
%     \item We use the simulation statistics generated from the simulation are used to     continually update the conditional probabilities of the system consequence, which is in turn used to update the system's operational risk.  
    
%     \item We demonstrate our approach using an \ac{av} example in CARLA simulation~\cite{dosovitskiy2017carla}.
% \end{itemize}

The paper is organized as follows. In \cref{sec:ps}, we formulate the problem. In \cref{sec:approach}, we describe the proposed risk-aware scenario generation approach. In \cref{sec:evaluation}, we apply our approach to an \ac{av} system in CARLA simulation. Finally, in \cref{sec:conclusion} we describe future extensions to our approach and conclude our work. 


% In \cref{sec:rw}, we provide a brief overview of existing work in the field of scenario generation for autonomous \acp{cps}.

==> Accepted/paper.tex <==
\section{Introduction}
The widespread use of autonomous \acp{cps}\footnote{CPS with \ac{lec}} has often required them to operate under uncertainties like sensor degradation and shifts in the operating conditions, which increase its operational risk. Design-time Assurance Cases~\cite{bishop2000methodology} and risk assessment are used to argue the system's safety at runtime. However, design-time information is inadequate for runtime estimations~\cite{denney2015dynamic} and a dynamic assurance approach is needed to handle the dynamically changing operating conditions in which the system operates. Dynamic Assurance requires designing runtime monitors like \ac{ood} detectors~\cite{sundar2020out} and dynamic assurance monitors~\cite{hartsell2021resonate} for estimating the system's risk of failure in the dynamically changing operating conditions. Designing these components often requires labeled data from scenes of failure conditions and corner cases in which the system fails. These scenes are referred to as risky scenarios~\cite{ma1999worst} or safety-critical scenarios~\cite{ding2020learning}; in this paper, we refer to them as high-risk scenes.

% The widespread use of autonomous \acp{cps}\footnote{CPS with \ac{lec}} has often required them to operate under uncertainties like sensor degradation and shifts in the operating conditions, which increase its operational risk. Design-time Assurance Cases~\cite{bishop2000methodology} and risk assessment are used to argue the system's safety at runtime. However, design-time information is inadequate for runtime estimations~\cite{denney2015dynamic} and a dynamic assurance approach is needed to handle the dynamically changing operating conditions in which the system operates. One approach to dynamic assurance is to measure the system's dynamic risk~\cite{hartsell2021resonate}. This requires designing runtime monitors like \ac{ood} detectors~\cite{sundar2020out} and risk estimators~\cite{hartsell2021resonate} for identifying operational scenes with a shift in the operating conditions, failure conditions, or corner cases in which the system fails. These scenes are commonly referred to as worst case scenarios~\cite{worstcaserl} or safety-critical scenarios~\cite{ding2020learning}; in this paper, we refer to them as high-risk scenes.


Similar to the \ac{ood} problem~\cite{cai2020real,sundar2020out}, often the data related to risky scenarios is under-represented in the training sets~\cite{khan2019striking}, leading to a data imbalance problem. If we can generate these under-represented events, they can be used to retrain the models to improve their accuracy~\cite{fremont2019scenic}. Further, such new scenes can be used for updating the machine learning components. However, collecting real-world data of such high-risk scenes can be expensive and slow in real-world conditions. There has been a growing interest in using synthetic data from simulators to address this problem~\cite{zhao2017accelerated,ma1999worst,dreossi2019verifai,viswanadha2021parallel}. For example, domain-specific \ac{sdl} like Scenic \cite{fremont2019scenic}, and MSDL \cite{msdl} provide probabilistic sampling capability integrated with CARLA \cite{dosovitskiy2017carla} to generate meaningful high-risk scenes. In addition, tools like Dakota~\cite{dalbey2021dakota} provide efficient sampling approaches like incremental sampling, importance sampling, and adaptive sampling and have been used for uncertainty quantification in engineering design.

Despite their success in generating high-risk scenes, we point to several limitations. First, the existing approaches perform \textit{passive sampling}, which does not use feedback from the previous results in the sampling process. Second, the scene variables being sampled typically have \textit{sampling constraints} and \textit{co-relations} that need to be considered. For example, the environmental properties of a scene (e.g., precipitation) may have physical constraints on their values that govern its temporal evolution. Applying these constraints is necessary for generating meaningful scenes~\cite{fremont2019scenic}. But the existing approaches do not include these sampling constraints. Third, conventional samplers do not balance the \textit{exploration vs. exploitation trade-off}. For example, random search and Halton search prioritizes uniform coverage of the search space, so they only explore. Whereas grid search aims to exhaustively cover a given grid, so they only exploit. However, as discussed by Jerebic, Jernej \emph{et al.}~\cite{jerebic2021novel}, balancing these strategies can result in higher coverage diversity which is commonly measured using clustering properties like the number of clusters and cluster population. 

To address these limitations, we present a scene generation approach that has a domain-specific \ac{sdl} integrated with two sampling approaches for generating high-risk simulation scenes. The key contribution of our work are two sampling approaches called \ac{rns} and \ac{gbo}. These samplers perform active sampling by using feedback of previous simulation results in the sampling process. They also include sampling constraints that govern the evolution of scene variables. In addition, they provide explicit hyperparameters to control the tradeoff between exploration vs. exploitation of the search strategy, using a novel risk-based scoring function. We demonstrate our approach using an \ac{av} case study in the CARLA simulator \cite{dosovitskiy2017carla}. To evaluate our samplers, we compared them against the baselines of random search, grid search, and Halton sequence search~\cite{halton1960efficiency} in terms of the total risk scenes, diversity, and search time metrics. Our experimental evaluation shows that the \ac{rns} and \ac{gbo} outperform the baselines in terms of the total risk scenes and diversity metrics. Also, the \ac{rns} sampler had comparable search times to the baselines, but the \ac{gbo} sampler has a higher search time. The source code and the technical appendix are available online\footnote{\label{github}https://github.com/scope-lab-vu/Risk-Aware-Scene-Generation-CPS}.

\begin{figure}[t]
 \centering
 \includegraphics[width=0.9\columnwidth]{figures/system-model3.pdf}
 \caption{\ac{av} system model designed for the CARLA autonomous challenge~\cite{carla-challenge}. The \ac{av} is primarily driven by an \ac{lec}-based navigation controller, which is supervised by an AEBS for emergency braking.} 
 \label{fig:sys-model}
\vspace{-0.1in}
\end{figure}

The outline of this paper is as follows. In \cref{sec:background}, we introduce the background on the typical design process and a dynamic assurance framework that we use. In \cref{sec:ps}, we describe the problem statement, followed by a description of our approach in \cref{sec:approach}. In \cref{sec:evaluation}, we implement and evaluate the samplers in the context of an \ac{av} case study in the CARLA autonomous driving challenge~\cite{carla-challenge}. This setup requires an \ac{av} (See \cref{fig:sys-model}) to navigate an urban town setting with complex traffic scenarios, adverse weather conditions, and sensor faults. Finally, we present related research in \cref{sec:rw} followed by conclusions in \cref{sec:conclusion}. 


\begin{figure*}[t]
 \centering
 \includegraphics[width=0.9\textwidth]{figures/btd.pdf}
 \caption{Bow-Tie Diagram for the \ac{av} case study adopted from our previous work~\cite{hartsell2021resonate}. Each block includes information about the event type and its description. The conditional probability and the threat $LUT$s are estimated from training data and discussed in \cref{sec:risk}.}
 \label{fig:btd}
\end{figure*}

==> Version1/abstract.tex <==
\begin{abstract}
Autonomous Cyber-Physical Systems must often operate under uncertainties like sensor degradation and distribution shifts in the operating environment, thus increasing operational risk. Dynamic Assurance of these systems requires augmenting runtime safety components like out-of-distribution detectors and risk estimators. Designing these safety components requires labeled data from failure conditions and risky corner cases that fail the system. However, collecting real-world data of these high-risk scenes can be expensive and sometimes not possible. To address this, there are several scenario description languages with sampling capability for generating synthetic data from simulators to replicate the scenes that are not possible in the real world. Most often, simple search-based techniques like random search and grid search are used as samplers. But we point out three limitations in using these techniques. First, they are passive samplers, which do not use the feedback of previous results in the sampling process. Second, the variables to be sampled may have constraints that need to be applied. Third, they do not balance the tradeoff between exploration and exploitation, which we hypothesize is needed for better coverage of the search space. We present a scene generation workflow with two samplers called Random Neighborhood Search (RNS) and Guided Bayesian Optimization (GBO). These samplers extend the conventional random search and Bayesian Optimization search with the limitation points. Also, to facilitate the samplers, we use a risk-based metric that evaluates how risky the scene was for the system. We demonstrate our approach using an Autonomous Vehicle case study in CARLA simulation. To evaluate our samplers, we compared them against the baselines of random search, grid search, and Halton sequence search. Our samplers of RNS and GBO sampled a higher percentage of high-risk scenes of 83\% and 92\%, compared to 56\% 66\% and 71\% of the grid, random and Halton samplers, respectively. 


 

% to identify shifts in the operating environment and estimate the likelihood of system failures.

% Data from these high-risk conditions is often not available during training. Also,

 

% samplers of RNS and GBO sampled a higher percentage of high-risk scenes of 83\% and 92\%, compared to 56\% of the traditional grid search sampler. 

 

% sequential search-based samplers that can efficiently generate high-risk simulation scenes. The two sampling approaches are Random Neighborhood Search (RNS) and Guided Bayesian Optimization (GBO). These samplers employ a sequential search strategy in which they use the system's earlier performances for strategically sampling the variables for the next scene. To facilitate the samplers, we use a novel performance metric called the safety score, which evaluates how risky the scene was for the system. We demonstrate our approach using an Autonomous Vehicle case study in CARLA simulation. Our samplers of RNS and GBO sampled a higher percentage of high-risk scenes of 83\% and 92\%, compared to 56\% of the traditional grid search sampler. 






% We also show that our samplers help reveal the critical risky scenes, which are often missed by the traditional samplers.

% So, it is critical to find these high-risk scenes for designing the safety components and periodically updating them to incorporate the knowledge of these high-risk scenes, which can improve the system's robustness.


\end{abstract}

\begin{IEEEkeywords}
Cyber-Physical Systems, Dynamic Assurance, Dynamic Risk, High-risk Scene, Bow-Tie Models, Hazards
\end{IEEEkeywords}

==> Version1/individual-sections/approach.tex <==
\section{Proposed Approach}
\label{sec:approach}
Overview of our approach is illustrated in \cref{fig:workflow}, and it consists of the following three broad components: (1) A scene generation approach designed using a \acl{sdl}. (2) A risk-based metric that is used to score the generated scenes. (3) The proposed sampling approaches called \acl{rns} and \acl{gbo}. We describe these components in detail below.  

\subsection{Scene Generation}
\label{sec:scene_generation}
We have designed a probabilistic scene generation language to generate scenes. The language includes a \acl{sdl} (SDL) integrated with probabilistic samplers to sample scenes over different scene variables introduced in \cref{sec:ps}. The \ac{sdl} has two components. (a) \textit{grammar}, which consists of a set of rules required to define the scene concepts in the meta-language. (2) \textit{meta-model}, which defines the concept of a scene using scene variables and their distribution ranges. In this setup, a scene $s$ = \{$e_1$,$e_2$,...,$e_i$\} is a collection of entities, where each entity is a three tuple $<s_v,v_d,v_c>$ of the scene variables $s_v$, distribution properties $v_d$ (e.g., distribution type, ranges) and variable constraints $v_c$. The language is designed using the textX \cite{dejanovic2017textx} meta-language. The language also has an interpreter to generate the scene artifact files and run the simulator. In addition, the interpreter abstracts the complexity of the language from the user by providing a scene specification file with scene variables and samplers that can be chosen to generate different scenes. The scene generation approach is illustrated in \cref{fig:workflow}.  


\subsection{Scoring Function}
\label{sec:scoring}
% We have designed a risk-based metric called the \textit{Risk Score} ($S_{Risk}$) to score the sampled scene. This score is a weighted combination of two utility functions $S_{Risk} =  w_1 \cdot RS + w_2 \cdot IS$. The utility functions are. (1) \textit{\ac{resonate} Score} ($RS$), which measures the system's dynamic risk in the scene using the likelihood hazard rates measured by \ac{resonate} discussed in \cref{sec:risk_estimation}. (2) \textit{Infraction Score} ($IS$), which measures the actual infractions (e.g., running a stop light) performed by the system. In this work, we used equal weights $w_1$ = $w_2$ = 1 for both these utility functions. We did this to ensure that both the estimated risk and the actual risk caused by actual infractions are equally weighted in the subsequently sampled scenes. 

We have designed a risk-based metric called the \textit{Risk Score} ($S_{Risk}$) to score the sampled scene. This score is a weighted combination of two utility functions as shown in \cref{eqn:risk_score}. The utility functions are. (1) \textit{\ac{resonate} Score} ($RS$), which measures the system's dynamic risk in the scene using the likelihood hazard rates measured by \ac{resonate} discussed in \cref{sec:risk_estimation}. (2) \textit{Infraction Score} ($IS$), which measures the actual infractions (e.g., running a stop light) performed by the system. In this work, we used equal weights $w_1$ = $w_2$ = 1 for both these utility functions. We did this to ensure that both the estimated risk and the actual risk caused by actual infractions are equally weighted in the subsequently sampled scenes. 



\begin{equation}
\label{eqn:risk_score}
    S_{Risk} =  w_1 \cdot RS + w_2 \cdot IS
\end{equation}


% In future work, we will vary these weights to see the impact on the kind of scenes that will be sampled. 

% The metric evaluates a scene based on the risk it poses to the system's safe operation. However, instead of only using the operational system risk that is estimated using the likelihood failure rates predicted by \ac{resonate}, we also include the actual system infractions in scoring a scene. So, the scoring function is a sum of the \textit{\ac{resonate} Score} ($RS$) and the \textit{Infraction Score} ($IS$). 

% Rather denote that there are two utility functions. One that measures RS and the other that measures IS. The overall utility function that you seek to maximize in the new samples is a weighted combination of both. You chose to provide same weight to both. This ensures that the scenes with both perceived risk and actual risks are equally weighted and identified in the future samples. In future it will be an interesting experiment to see what happens if you change these weights.

% While $RS$ provides the average likelihood of the system consequence across the scene, $IS$ provides the actual system infractions. 

% \begin{equation}
% \label{eqn:safe_score}
%     S_{Risk} =   \ac{resonate} \; Score + Infraction \; Score
% \end{equation}
% uses the design-time probabilities of the \ac{btd} event along with runtime measurements from monitors like anomaly detectors and \ac{ood} detector to

\subsubsection{\ac{resonate} Score ($RS$)} Measures the average risk of the system's consequence across the scene. To compute this score, we leverage the \ac{resonate}~\cite{hartsell2021resonate} risk estimator which estimates the dynamic hazard rate $\lambda$ at every time step. The hazard rates are averaged across the scene using $\frac{\int_{T_1}^{T_2} \lambda \,dt}{T_2-T_1}$, where $\lambda$ is the estimated hazard rate and $T_1$, $T_2$ are the start and end time of the scene, to compute the system's dynamic risk or the \ac{resonate} score. In this work, our simulations are typically $1$ minute long, so $T_1$=0 and $T_2$=1 are used in the calculations.

\subsubsection{Infraction Score ($IS$)} Measures the system's actual infractions in the simulator. This score can include a variety of infractions like route deviation, lane violation, and traffic rule violation. These infractions ($I_k$) can be weighted ($w_k$) according to their severity and later summed together to compute the infraction score $IS$ = $\sum_{k=1}^{n} w_k \cdot I_k$ 


% \begin{equation}
%     Infraction \; Score = \sum_{k=1}^{n} w_k \cdot I_k
% \label{eqn:driving_score}
% \end{equation}
For example, the infraction score for the \ac{av} case study (See \cref{sec:casestudy}) was computed as $IS = 0.7 \cdot I_S + 0.8 \cdot I_R + I_{RD}$. Where $I_S$ is running a stop sign infraction, $I_R$ is running a red-light infraction, and $I_{RD}$ is the deviation in the route taken by the \ac{av}. These weights are chosen specifically for the case study. Finally, we compute $S_{Risk}$ using these two scores.

% For the \ac{av} case study, we have used the weighted sum of the Infraction penalties ($I$) and the Route Deviation ($I_{RD}$) metrics as $IS = 0.7 \cdot I_S + 0.8 \cdot I_R + I_{RD}$.

% An example of these infractions for two different scenes is shown in \cref{fig:hazard_rate}.  

% \begin{figure}[t]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/hazard-rate.pdf}
%  \caption{The estimated collision rate for two test scenes. (Top) Scene1 - A scene with two camera faults. The average collision rate across the scene was $0.4$ and the infraction score was $0$ (Bottom) Scene2 - A scene with adverse brightness. The average collision rate across the scene was $0.69$ and the infraction score was $0.15$.}
%  \label{fig:hazard_rate}
%   \vspace{-0.15in}
% \end{figure}

Now, a scene with $S_{Risk}$ $>$ $\delta$ is classified to be high-risk. $\delta$ is the risk threshold computed across the previously encountered calibration scenes. Considering these scenes are sampled from the same underlying distribution, we 
select a simple threshold at the $95^{th}$ percentile ($2$ standard deviations) of $S_{Risk}$ for every scene in the calibration set. 

% Now, for classifying the scene as high-risk, we calculate a risk score threshold $\delta$ across all the previously encountered scenes. This threshold is calculated across a part of the calibration set, which is not used for designing the risk-estimator. This set includes scenes with sensor faults and adverse brightness along with the normal scenes from training. Now, as these scenes are sampled from the same distribution, we use $2$ standard deviations ($\mu$ + $2\cdot\delta$) of the $S_{Risk}$ score across the calibration set as the threshold. In our setup, any scene that has $S_{Risk}$ $\geq$ $\delta$ is classified to be of high-risk.

\input{results/rns}

\subsection{Sampling Approaches}
\label{sec:samplers}
We present two samplers called the \acl{rns} and \acl{gbo}, which are extensions of the conventional random and \ac{bo} search. The extensions are. (1) \textit{active sampling}, we use a feedback loop of previous simulation results to sample the next scene variables. (2) \textit{constraints-based search}, we create sampling constraints $\mathcal{SC}$ to add constraints on the scene variables. \cref{Table:constraints} shows the constraints that we applied for an \ac{av} case study. (3) \textit{exploration vs. exploitation trade-off}, we introduce explicit hyper-parameters to balance the strategies.


% \input{results/sampling_rules}


\subsubsection{Random Neighborhood Sampler (RNS)}
This sampler extends the conventional random search by including the kd-tree nearest neighborhood search algorithm~\cite{friedman1975algorithm}. With this extension, we aim to add the missing exploitation capability to random search. Briefly, the approach works as follows. It initially explores a scene through random sampling and then exploits the area around the explored scene using the sampling constraints and the nearest neighbor search. \cref{algo:rns} illustrates the steps involved, and it works as follows. 

\textit{First}, the algorithm explores the search space $\mathcal{D}$ by randomly sampling the scene variables $s_v$ from their respective distributions $V_D$. These randomly selected variables are used to generate the scene artifact files, run the simulator and compute the risk score $S_{Risk}$ for the scene. The randomly generated scene is represented as $R$ in \cref{fig:workflow}.

\textit{Second}, if the $S_{Risk}$ $<$ $\delta$, the simulation run statistics are stored, and the scene variables are again randomly sampled from the search space $\mathcal{D}$. However, if the $S_{Risk}$ $>$ $\delta$, the neighborhood around the randomly sampled scene $R$ is exploited to generate more scenes. For this, we use the sampling constraints $\mathcal{SC}$ shown in \cref{Table:constraints}. These constraints will create a bounded region $\mathcal{B}$ around $R$ from which the subsequent scene variables are randomly sampled. 

\textit{Third}, the algorithm uses the kd-tree nearest neighborhood search to find if there are at least $k$ scenes generated in the neighborhood of the explored scene $R$. That is, it checks if $R$ has at least $k$ similar scenes in $\mathcal{E}$. To measure the similarity, we use the $l_2$ distance metric $(d(x,R) = ||x - R||_2)$ and identify the similar scenes as $N = \{\forall s \in \mathcal{E}| d(R,s_i) < \tau \}$. Where $R$ is the currently sampled scene and $s_i$ are scenes in the previously explored list $\mathcal{E}$. This step returns a list of neighbors whose distances to $R$ are smaller than a threshold $\tau$.  If the number of the neighbors $N$ $\geq$ $k$, the search around $R$ is stopped. Then,  step1 is performed to randomly explore a new scene in the entire search space $\mathcal{D}$. However, if $N$ $\leq$ $k$, then the search around $R$ is continued. In this sampler, $k$ is the hyperparameter used to control the exploitation.


% using the following equation. 

% \begin{equation}
% \label{eqn:distance}
%     N = \{\forall s \in \mathcal{E}| d(R,s_i) < \tau \}
% \end{equation}

\input{results/bo}

\textbf{Limitation:} Although the sampler can both explore and exploit the search space, the exploration is performed uninformed without strategic knowledge about the search space. This could result in high-risk regions of the search space left unexplored.

\subsubsection{Guided Bayesian Optimization (GBO)}
\label{sec:gbo_sampler}
The uninformed exploration problem of the \ac{rns} is addressed by this sampler, which is an extension to the conventional \acl{bo}. To perform informed exploration and active sampling, the algorithm has two components. The first component is a probability function model that is fitted across all the previously explored variables. This feedback allows the model to learn the region of the search space that has large uncertainty that will return a higher objective value. A \ac{gp} model is most used to fit the function. The second component is an acquisition function that strategically finds the succeeding variables, which will optimize the objective function. We use the \ac{ucb}~\cite{auer2002using} acquisition function that provides the $\beta$ hyperparameter to control the exploration vs. exploitation trade-off (See \cref{eqn:ucb}). Finally, to these components, we include sampling constraints. \cref{algo:bo} shows the operation of the \ac{gbo} sampler, which is discussed below. 

\textit{First}, the \ac{gp} model with properties $\mu$[0] and $\sigma$[0] is initialized for first k iterations. During these iterations, the scene variables $s_v$ are randomly sampled from the input search space $\mathcal{D}$. These randomly sampled variables are used to generate scene artifact files and run the simulation. Then, $S_{Risk}$ is computed and added to the exploration list $\mathcal{E}$ along with the sampled variables. After the k initial iterations, the initialized \ac{gp} model is fitted across all the entries in $\mathcal{E}$ to calculate new posterior distribution $f(x_n)$ with updated $\mu$[$x_n$] and $\sigma$[$x_n$]. 

% . Then, the marginalization property of the \ac{gp} model allows for the calculation of a new posterior distribution $f(x_n)$ with an updated posterior mean $\mu$[$x_n$] and $\sigma$[$x_n$]. 

\textit{Second}, the algorithm uses the sampling constraints $\mathcal{SC}$ to create a smaller search space $\mathcal{B}$ in which the acquisition function will sample the succeeding variables. \textit{Third}, the updated posterior distribution properties and the bounded search space created by the sampling constraints are used by an acquisition function to strategically select the variables for the next scene that will optimize $S_{Risk}$. In this work, we use the \ac{ucb} \cite{auer2002using} as the acquisition function, which is given below. 
 
\begin{equation}
\label{eqn:ucb}
    x_{n+1} = \argmax\limits_{x \in \mathcal{D}}\mu[x_n] + \beta^{1/2} \cdot \sigma[x_n]
\end{equation}

Where $x_{n+1}$ are the newly selected variables that have the largest \ac{ucb}. $\mu[x_n]$ and $\sigma[x_n]$ are the properties of the updated \ac{gp} model. $\beta$ is a parameter that allows for exploitation and exploration tradeoff. A larger value of $\beta$ allows for higher exploration, and a lower value allows for exploitation. So, $\beta$ needs to be carefully selected for optimizing the balance of the two strategies. 
Next, the newly sampled variables are used to generate the scene artifact files, which run the simulation. Then, $S_{Risk}$ is computed and added to the list $\mathcal{E}$ along with the selected variables. The steps of the algorithm are repeated for a specified number of iterations $t$.  

\textbf{Limitation:} The sampler has two problems that arise because of using the \ac{gp} model. (a) Cold-start, which requires the model to be trained from scratch each time the sampler is used. This increases the sampling time. To address this, we use the knowledge of randomly sampled scenes from the previous runs to ``warm start" the search process. (b) Scalability, the \ac{gp} model suffers from a cubic time complexity~\cite{liu2020gaussian}, which limits its applicability to a large number of executions. To address this, we will use a scalable \ac{gp} model in the future.  





==> Version1/individual-sections/background.tex <==
\section{Background}
\label{sec:background}
% In this section, we introduce the Dynamic Assurance topics that are required to understand our approach.
% - explain what you assume about system design procedures.
% - background on dynamic assurance.
% - explain BTD


\subsection{System Design Procedures}
We assume that the \ac{cps} undergoes design, training, and deployment activities categorized into four steps: (1) \textit{Design Phase}, which involves system analysis, hazard analysis, and Assurance Case construction. (2) \textit{Training Phase}, which involves collecting training scenes and training the \ac{lec} controllers on these scenes. (3) \textit{Calibration Phase}, which involves designing and calibrating the anomaly detectors, \ac{ood} detectors ~\cite{cai2020real,sundar2020out} and dynamic assurance monitors (\cref{sec:risk_estimation}). Estimating the system risk requires curating a calibration set that includes scenes with sensor faults and adverse operating conditions in addition to the training scenes. (4) \textit{Testing Phase}, which involves generating high-risk test scenes for testing the trained system.

%We briefly describe these steps and expectations below.

In particular, the design phase is important because it consists of gathering and documenting information about the system's top-level goals, requirements, system operating conditions, and system faults. It also includes designing the system models including, architecture model (e.g., \cref{fig:sys-model}), and system function breakdown.  Thereafter, we assume that the designers perform \textit{Hazard Analysis}, which involves identifying the hazards to the system that will result in a system consequence. The system could have a collection of hazards $\{H_1, H_2,\cdots, H_n\}$ stemming from its operation, functioning, software components, hardware components, etc. Any of these hazards in a given condition can result in a system consequence. This enables creation of \ac{btd}~\cite{ferdous2013analyzing}, a model describing the chain of events $t_i \rightarrow b_p \rightarrow e_{top} \rightarrow b_m \rightarrow c_i$, where $t_i$ are system threats, $b_p$ are preventive barriers, $e_{top}$ is a top event, $b_m$ is a mitigation barrier, and $c_i$ is a system consequence. Fig \ref{fig:btd} describes the operational hazard of ``roadway obstruction'' for the \ac{av} case study (\cref{fig:sys-model}). The \ac{btd} has two system threats: vehicles (T1) and pedestrians (T2) in the path of the ego vehicle. These threats can escalate to become a top event (TOP) if preventive barriers of $B1$ and $B2$ are not introduced. The performance of the perception \ac{lec} is used as the barrier. If the perception LEC fails, then the roadway hazard can become a safety consequence $C1$ if not mitigated by a barrier of $B3$, the emergency braking system.  During the design, these hazard analyses are used to create assurance cases~\cite{bishop2000methodology}, showing that the top-level goals of the system are satisfied. Further, such hazard diagrams enable the system to be dynamically monitored for the likelihood of failures through a technique called dynamic assurance. 

     
 \iffalse   
 The \textbf{training} phase consists of developing the  \ac{lec}s. The 
    \item \textbf{Training Phase}: We assume the training phase consists of the data collection and the design and training of the \ac{lec}s. These components are mostly deep neural networks that are often trained through supervised learning~\cite{hastie2009overview} or reinforcement learning~\cite{sutton2018reinforcement}. The training process is often cumbersome with several hyperparameters to tune (e.g., model architecture layers, training epochs, batch size). Tool-chains like ALC~\cite{hartsell2019model} assist the hyperparameter selection and training process. 
    
    % \textcolor{red}{please put citations - like our ALC papers}
    
   
    \item \textbf{Calibration Phase} : We assume the calibration phase consists of designing and calibrating runtime monitors for dynamic assurance.
    %Along with conventional anomaly detectors for detecting software and hardware anomalies, it is required to consider the uncertainties of \ac{lec}s for \acl{ood} scenes.
    Detecting the \ac{ood} data problem requires designing complex anomaly detectors called \ac{ood} detectors or assurance monitors~\cite{cai2020real,sundar2020out}. Finally, estimating the system risk also requires designing risk estimators~\cite{hartsell2021resonate} (e.g. \cref{sec:risk_estimation}). %These monitors are trained and calibrated using the training data.   
    
    % \textcolor{red}{put citations of xenofon, penn and berkley and other papers}
    
   % Describe OOD detectors and other monitors trained
    \item \textbf{Operational Phase}: We assume at runtime, the trained \ac{lec} with the calibrated runtime monitors are used for operating the system. At each time step, the \ac{lec} predicts the control actions for the system, and the runtime monitors detect any outliers in the sensor measurements or changes in the operating conditions. The results from these runtime monitors can be used to assess the dynamic risk to the system using a dynamic assurance framework. 
    %    are often used for high-level controller selection~\cite{zakharov2015performance} based upon  
    
    % During the runtime, dynamic assurance framework is deployed -- summarize
\end{enumerate}
\fi
%\textbf{Operational Phases}:We classify the design, training, and deployment activities into $4$ phases as shown in \cref{fig:workflow}. They are. (1) \textit{Design Phase}, which involves system analysis, hazard analysis, and Assurance Case construction. (2) \textit{Training Phase}, which involves collecting training scenes and training the \ac{lec} controllers and the anomaly detectors on these scenes. (3) \textit{Calibration Phase}, which involves designing and calibrating the risk estimator. Estimating the system risk requires curating a calibration set that includes scenes with sensor faults and adverse operating conditions in addition to the training scenes. (4) \textit{Testing Phase}, which involves generating high-risk test scenes for testing the trained system.

% The system can have several top level goals adhering to different properties of the system like safety, security, functional, etc.
\iffalse
\textbf{1) System Analysis} involves gathering and documenting information about the system's top-level goals, requirements, system's operating conditions, and system faults. It also includes designing the system models including, architecture model (e.g., \cref{fig:sys-model}), and system function breakdown. 

\textbf{2) Hazard Analysis} involves identifying the hazards to the system that will result in a system consequence. The system could have a collection of hazards $\{H_1, H_2,\cdots, H_n\}$ stemming from its operation, functioning, software components, hardware components, etc. Any of these hazards in a given condition can result in a system consequence. A \ac{btd} \textcolor{red}{cite BTD} is a graphical structure that is often designed to analyze the hazard propagation and identify the possible control strategies to prevent the hazard from failing the system. The \ac{btd} can be represented as a chain of events $t_i \rightarrow b_p \rightarrow e_{top} \rightarrow b_m \rightarrow c_i$. Where, $t_i$ are system threats, $b_p$ are preventive barriers, $e_{top}$ is a top event, $b_m$ is a mitigation barrier, and $c_i$ is a system consequence. To explain these events, consider the \ac{btd} (See \cref{fig:btd}) for an operational hazard of ``roadway obstruction" for an \ac{av} case study that is introduced later in \cref{sec:casestudy}. To explain the \ac{btd}, it has two system threats of vehicles (T1) and pedestrians (T2) in the travel paths, which is derived from hazard analysis. Now, these threats can escalate to become a top event (TOP) if preventive barriers of $B1$ and $B2$ are not introduced. In this case, the performance of the \ac{lec} is used as the barrier. Next, the top event could escalate to become a consequence not mitigated by a barrier of $B3$. In this example, the performance of AEBS in emergency braking is selected as the barrier. 

\textbf{3) Assurance Case Construction} involves using the system and hazard analysis information to construct an assurance case~\cite{bishop2000methodology}, which can argue using the available system evidence that the top-level goals of the system are satisfied.   

% to handle dynamically changing operating conditions in which these systems operate
\fi
\subsection{ReSonAte}
\label{sec:risk_estimation}
%Design-time information is  used to assure the system properties (e.g., safety, security) at runtime. However, 

%Static assurance cases  are not very accurate because the system hazards can be dependent on the operating conditions and the system state~\cite{denney2015dynamic}. 
%For example, a hazard (e.g., camera blur) that is of high consequence in one operating condition (e.g., night) can have a low consequence in the other (e.g., day). To capture this,
%The dynamic assurance approach  uses runtime measurements in addition to the static assurance cases to estimate the ``system's dynamic risk". %
%\ac{resonate}~\cite{hartsell2021resonate} is an example of dynamic assurance framework.



%with the design-time information is required. Our approach to dynamic assurance is to estimate the ``system's dynamic risk". 
%\textbf{ReSonAte:} To perform dynamic risk estimation, we leverage our previously developed tool called \ac{resonate}~\cite{hartsell2021resonate}. The tool uses the 
%\ac{btd} to estimate the dynamic hazard rate $\lambda$ for every hazard that is identified in the design phase. The hazard rate can be used to compute the likelihood of the hazard occurrence in a given time unit $1-e^{-\lambda \cdot t}$, where $\lambda$ is the estimated hazard rate, and $t$ is the duration..
%The likelihood of different hazards contributes to the system's risk. 

% In this setup, we consider the likelihood of different hazards to be independent.
 
% The system can have several hazard rates stemming from different hazardous failures. These rates put together constitute the system's risk. For estimating $\lambda$, \ac{resonate} uses a hazard propagation structure called \ac{btd}. Designing the \ac{btd} is a design-time activity, which begins with hazard analysis, which includes identifying the events to the system like Threats (T), which may lead the system into a hazard (H), and the possible barriers (B) to prevent the hazard from propagating into a consequence. These hazard events are used to design a \ac{btd}, which is often used to visualize hazard propagation, identify control strategies, and estimate the system's risk.  

\ac{resonate} ~\cite{hartsell2021resonate} uses an augmented \ac{btd} (derived from the hazard analysis). The augmentation adds various event probabilities for each causal chain, conditioned on the state of the system and the environment, including sensor failures, actuator failures, and output of \ac{ood} detectors and environmental conditions. Specifically, it requires estimation of the (a) the conditional probability of the barrier's success in each state $(f_b(x=B_i),s)$, and (b) the frequency of occurrence of a threat $f_e(T_i,s)$ in each state. These conditional relationships must be inferred from data and are often inferred by using the observation of system's and barrier's performance across various scenes. For this, we use the calibration set collected using a grid sampler, where we select the conditions affecting the barrier and generate scenes around it. The estimated probabilities are stored in \acp{lut} as illustrated in \cref{fig:btd}. At runtime, the \acp{lut} is used to identify the current context and then identify the hazard rate for the consequence ($\lambda$). The hazard rate can then be used to compute the likelihood of the hazard occurrence in a given time unit $1-e^{-\lambda \cdot t}$, where $\lambda$ is the estimated hazard rate, and $t$ is the duration.

%The hazard rate is estimated using a \ac{btd}, and it requires calculating the probabilities of the different events in the \ac{btd}. The probabilities that are of interest are. (a) the conditional probability of the barrier's success in each state $(f_b(x=B_i),s)$. and (b) the frequency of occurrence of a threat $f_e(T_i,s)$ in each state. This term gives the expected frequency of threat in units of the expected number of occurrences in a given time interval. Also, it is important to note that these probabilities may be conditionally dependent on the system's state ($s$) including sensor failures, system failure modes, anomaly detectors, and environmental conditions. To model conditional dependence, we need to identify the conditions relevant to the barriers. These conditional relationships must be inferred from data. For this, we generate a calibration set using a grid sampler, where we select the conditions affecting the barrier and generate scenes around it. The estimated probabilities are stored in \acp{lut} as illustrated in \cref{fig:btd}, and their calculations are discussed in \cref{sec:evaluation}. 

%Now, these probabilities are used with runtime measurements from detectors to estimate the dynamic hazard rate and the system's dynamic risk. We refer to this dynamic risk as to the \ac{resonate} score in this paper. Along with conventional anomaly detectors to identify outliers in sensor measurements and software components, it is required to consider the uncertainties introduced by the \ac{lec}s because of the \acl{ood} conditions. This requires designing complex anomaly detectors called \ac{ood} detectors~\cite{sundar2020out}. 

% Now, estimating this score requires designing anomaly detectors to identify outliers in sensor measurements and software components.  Also, it is required to consider the uncertainties introduced by the \ac{lec}s because of the \acl{ood} conditions. This requires designing complex anomaly detectors called \ac{ood} detectors~\cite{sundar2020out}. 





% \subsection{CPS operational Phases}
% To perform dynamic assurance of autonomous \ac{cps}, we classify the design, training and deployment activities into the following phases. (1) \textit{Design Phase} involves system analysis, hazard analysis and construction of an Assurance Case. (2) \textit{Training Phase} involves collecting training scenes and training the \ac{lec} controllers and the anomaly detectors on these scenes. (3) \textit{Calibration Phase} involves designing and calibrating the risk estimator. Estimating the system risk requires curating a calibration set that includes scenes with sensor faults and adverse operating conditions in addition to the normal training scenes. (4) \textit{Testing Phase} involves generating high-risk test scenes for testing the trained system.

% which the system has high operational risk and is susceptible to fail. 

% designing and modeling the system, identifying the system operating conditions, identifying the system hazards, sensor faults, and finally designing an Assurance Case.


% using the proposed samplers to generate high-risk scenes for testing the trained \ac{lec} and the safety components. In the future, we will use the generated high-risk scenes to iteratively update the controller and the safety components. 



==> Version1/individual-sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented a scene generation approach that integrates a \acl{sdl} with two samplers and a risk-based scoring function for generating high-risk scenes. The proposed samplers are \acl{rns} and \acl{gbo}. These samplers are based on the conventional random and \ac{bo} search techniques, and we add capabilities of active sampling, constraint-based sampling, and balancing the exploration vs. exploitation to guide them towards sampling clusters of high-risk scenes. We applied these samplers to an \ac{av} case study. Our evaluations show that the proposed samplers could sample a higher number of high-risk scenes that could be clustered into a higher number of clusters as compared to the conventional baselines. 

% There are many directions for future work. (1) Parallelize the sampling approaches across multiple systems under test. (2) Continually update the controller, detectors, and the risk estimator with the recently generated scene samples. (3) Try policy-based \ac{rl} for generating a sequence of scenes that can maximize the system's risk.
\textbf{Acknowledgement}: This work was supported by the DARPA Assured Autonomy project and Air Force Research Laboratory. 


% Also, we have designed a novel scoring function to score the scenes and guide the samplers. We demonstrate this workflow for an \ac{av} example in CARLA simulation. Our samplers outperformed the baselines in terms of the total risk scenes, diversity, and search time metrics.

% extend the conventional random search and \ac{bo} search with additional capabilities

% Future extensions of the approach include. (1) \acl{rl} sampler to generate a sequence of scenes that pose high-risk to the system, (2) perform continual learning of the models as smaller batches of high-risk scenes rather than a single update at the end of testing phase. 

% Further, the high-risk scenes generated by the samplers are used to periodically update the system models to avoid concept drift and model staleness.

==> Version1/individual-sections/evaluation.tex <==


% \footnote{\label{github}source code to replicate the CARLA experiments can be found at \url{https://github.com/Shreyasramakrishna90/Risk-Aware-Scene-Generation}}

\section{Evaluation}
\label{sec:evaluation}
We evaluate our approach using an \ac{av} example in CARLA simulator~\cite{dosovitskiy2017carla}. The experiments were performed on a desktop computer with AMD Ryzen Threadripper 16-Core Processor, 4 NVIDIA Titan Xp GPU's and 128 GiB RAM memory.



\subsection{\ac{av} Case Study}
\label{sec:casestudy}

We have designed an \ac{av} the CARLA autonomous driving challenge~\cite{carla-challenge}, which is needed to navigate through an urban environment with adverse weather conditions and sensor faults while avoiding collisions with vehicles and pedestrians in its travel path. The simulator also offers individual metrics to measure the infractions caused by the system. The details of the system setup are discussed below.  

\subsubsection{System Model} The system block diagram of the \ac{av} is shown in \cref{fig:sys-model}. It uses a total of $9$ sensors including, three forward-looking cameras, two radars, an \ac{imu}, a \ac{gps}, and a speedometer. It has a \ac{lec} based navigation controller, which is adapted from Chen et al.~\cite{chen2020learning}. This controller uses a navigation planner that takes the waypoint information from the scene artifact file generated by our scene generation approach and divides the distance between the waypoints into smaller position targets. Then, it uses the \ac{gps} and \ac{imu} sensors to get the vehicle's current position and the next position to reach. Next, the position information is fed into a velocity planner to compute the vehicle's desired speed. The desired speed and camera images are fed into a perception \ac{lec}, which predicts the throttle and steering angle errors. These signals are sent to PID controllers to compute the throttle, brake, and steer control signals. Besides the \ac{lec}, there is also an \ac{aebs}, which uses the radar estimated object distance ($r_d$) with the vehicle's current speed to compute a ``safe braking distance" ($b_d$). If $r_d \leq b_d$, a brake alarm is issued. The alarm overrides the throttle signals from the \ac{lec}. Finally, these control signals are sent to the simulator. 

\subsubsection{System Operational Phases} The \ac{av} is operated in the following phases. In the \textit{Design phase}, we designed the system model (See \cref{fig:sys-model}) and performed a primary hazard analysis. In this work, we restricted the hazard analysis to identify operational threats to the \ac{av}. Finally, we identified the sensor faults that fail the system. For the \ac{av}, we found camera blur and occlusion affected the perception \ac{lec}. In the \textit{Training phase} we used the \ac{av}'s autopilot controller~\cite{chen2020learning} to drive around randomly generated scenes to collect data for training the \ac{lec} controller. Next, in the \textit{Calibration phase}, we calibrate the \ac{ood} detector and the \ac{resonate} risk estimator. For risk estimation, we compute the \ac{btd} probabilities using the calibration set, which included scenes from the training set and additional scenes with sensor faults and adverse weather conditions, collected using a grid sampler. Finally, in the \textit{Testing Phase}, the trained \ac{lec} and the monitors are tasked to operate in $250$ scenes generated by the proposed samplers.   


% \begin{minipage}[!htb]{0.95\columnwidth}
% \centering
% \begin{minipage}{0.25\columnwidth}
% \begin{figure}[H]
%         \input{results/scene}
% \end{figure}
% \end{minipage}
% \hspace{0.28\columnwidth}
% \centering
% \begin{minipage}{0.4\columnwidth}
% \begin{figure}[H]
%         \input{results/faults}
% \end{figure}
% \end{minipage}
% \footnotesize
% \centering
% % \setlength{\abovecaptionskip}{2pt}
% \captionof{figure}{(left) Simulation Variables and their distribution ranges. (right) types of sensor faults considered in these scenes.}
% \label{Table:variables}
% \vspace{0.15in}
% \end{minipage}

\begin{figure*}[t]
 \centering
 \includegraphics[width=0.95\textwidth]{figures/simulation-scene4.pdf}
 \caption{Screenshots of different scenes generated for the CARLA \ac{av} case study. The description of these scenes are provided below the images.}
 \label{fig:scenes}
%   \vspace{-0.15in}
\end{figure*}



\subsubsection{Operating Scenes} As illustrated in \cref{fig:scenes}, our scenes included varying the weather conditions (cloud (C), precipitation (P)), time-of-day (T), traffic densities (TD), road segments (RS), and sensor faults (F). The distribution ranges of these scene variables are listed in \cref{Table:constraints}. Also, we applied the constraints on these variables while sampling. The constraints are listed in \cref{Table:constraints} and is discussed in \cref{sec:ps}. 

% To remind, the road segment has constraints on the distance between two consecutive waypoints. Also, the weather variables have constraints on how much their values can change between consecutive scenes. Traffic density is a special case that had constraints on its values, and it is also dependent on the type of road segments. Finally, camera blur and occlusion are the two faults that are injected into the three cameras on the vehicle.   


% \cref{fig:sampling-rules} while sampling these variables. 

% The structural variables of road segments and traffic density had constraints that were defined by the CARLA map. For example, the sub-rages for traffic were selected based on the vehicle's location (e.g., crossroads, intersections). The temporal variables had the constraint $n$ (see \cref{fig:sampling-rules}) on the rate at which its value changes. For this example, the value of $n$ = 5 was chosen. In addition, \cref{Table:variables} shows the sensor faults that we synthetically injected into the vehicle. 

% Also, we add Gaussian noise to the distances returned by the radar. 


% \begin{figure}[!t]
%  \centering
%  \includegraphics[width=\columnwidth]{figures/scene-variables.pdf}
%  \caption{(left) Simulation Variables and their distribution ranges. (right) types of sensor faults considered in these scenes.}
% \label{Table:variables}
% \vspace{-0.1in}
% \end{figure}


\subsubsection{Detectors} 
\label{sec:safety_components}
% To augment safety into the vehicle, we equipped it with several anomaly detectors and an \ac{ood} detector. 
To detect camera-related faults such as blurred images and occluded images, each of the three cameras is equipped with OpenCV based blur detector and occlusion detector. The blur detector uses the variance of the Laplacian operator~\cite{pech2000diatom} to measure the blur level in the images. A high variance shows that the image is not blurred, and low variance ($<50$) shows the image is blurred. The occlusion detector is designed to identify large blobs of continuous black image pixels. In our setup, if an image has connected black pixels $>10\%$, then the image is said to be occluded, otherwise, it is not. We empirically selected these thresholds based on the calibration set. For these images, the blur detectors and the occlusion detectors had an F1-score of 97\% and 98\%.  

In addition, we designed a reconstruction-based $\beta$-VAE \ac{ood} detector~\cite{sundar2020out} to identify shifts in the operating scenes. The detector model has four convolutional layers $16/32/64/128$ with (3x3) filters and (2x2) max-pooling followed by four fully connected layers with $2048$, $1000$, and $250$ neurons. It also has a symmetric deconvolutional decoder structure and hyperparameters of $\beta$=1.2 and latent space=$100$. We trained the model for $150$ epochs using the $6000$ center camera images. We tested it by synthetically introducing brightness into the training images. For these images, the detector had an F1-score of 98\%. At runtime, the reconstruction mean squared error of the detector is used with Inductive Conformal Prediction \cite{shafer2008tutorial} and power martingale \cite{fedorova2012plug} to compute a martingale value. We use the martingale value with a threshold of $20$, empirically selected for \ac{ood} detection. 

\begin{figure*}[t]
 \centering
 \includegraphics[width=0.95\textwidth]{figures/sampler-plots2.pdf}
 \caption{Comparison of the $250$ scenes sampled by the different samplers. While random and Halton samplers only explore the space, grid sampler only exploits the specified grid. In comparison, our samplers can both explore and exploit. This is evident from the dense scene clusters.}
 \label{fig:sampler_3d}
% \vspace{-0.1in}
\end{figure*}


\subsubsection{Risk Score}
\label{sec:risk}
To compute $S_{Risk}$, we first computed the \textbf{\ac{resonate} score} using the \ac{btd} with the hazard of ``roadway obstruction" shown in \cref{fig:btd}. To compute the collision rate $\lambda$, we analyzed the conditional relationships of \ac{btd}'s barriers and threats using the calibration set. The probability function of barriers $B1$ and $B2$ are dependent on the continuous-valued output of the \ac{ood} detector and the binary state of the anomaly detectors, which is captured using the following equation.

% . These relationships are captured using the following equation.

%  For this, we used the calibration set with normal scenes and scenes with different weather conditions and sensor failures, as discussed earlier.


\small
\begin{gather}
f_b(x=(B_1,B_2),s) = (1-P(x|s.m.LEC)) * \prod_{d\epsilon S^{B2}}{\frac{P(x|d)}{0.4} * f_{s}} \nonumber \\
P(x|s.m.LEC) = (1+e^{-0.049*(t.m.LEC-5.754)})^{-1}
\label{eqn:conditional_prob}
\end{gather}
\normalsize

Where, $P(x|s.m.LEC)$ is a sigmoid function used to capture the continuous values of the \ac{ood} detector, the discrete-valued probability of the anomaly detectors that constitutes the state-variables in $S^{B2}$. In our example, $B1$ and $B2$ were affected by the image quality, which we detect using the blur and occlusion detectors whose probabilities are reported in~\cref{fig:btd}. Also, $f_{s}$ is the failure rate of the sensors, which is assumed to be constant for both the camera and the radar sensors on which the barriers are dependent. Further, the probability function of $B3$ is conditionally dependent on the precipitation levels and the operation of the radar as shown in \cref{fig:btd}. These conditional relationships were inferred by clustering the calibration scenes based on the precipitation levels. In a similar approach, we also estimated the frequency of threat occurrence. In this example, the frequency of threats $T1$ and $T2$ was dependent on the road segments. That is, an intersection had a higher frequency of threats as compared to a side road. This information was aggregated from the calibration data and stored in a \ac{lut}. Finally, we used the hazard rates and the conditional probabilities to compute the dynamic collision rates and the system's dynamic risk or \ac{resonate} score as discussed in \cref{sec:scoring}.  

Next, we computed the \textbf{Infraction score} from the simulator statistics $IS = 0.7 \cdot I_S + 0.8 \cdot I_R + I_{RD}$. Where $I_S$ is running a stop sign infraction, $I_R$ is running a red-light infraction, and $I_{RD}$ is the deviation in the route taken by the \ac{av}. This score was added to the \ac{resonate} score to compute the $S_{Risk}$. Finally, we also computed the threshold $\delta$ to be $0.65$, as discussed in \cref{sec:scoring}. 

\subsection{Baselines and Competing Metrics} We compare our sampler to state-of-the-art techniques. The baselines that we compare against are. \textbf{1) Random Search} is a technique in which the scene variables are sampled uniformly at random from their respective distributions. \textbf{2) Grid Search} is a technique that exhaustively samples all the combinations of the scene variables in a given grid. \textbf{3) Halton Sequence Search}~\cite{halton1960efficiency} is a pseudo-random technique that samples the search space evenly using co-prime as its bases. We compare these baselines using the following metrics, which align with the two desirable sampler objectives discussed in \cref{sec:ps}. 

\textbf{1) Total Risk Scenes (TRS)}: The proportion of the high-risk scenes sampled to the total number of scenes sampled.
\begin{equation}
\label{eqn:rsp}
\small
    TRS (\%) = \frac{1}{N}\sum_{i=1}^{N} s_i \quad \textnormal{if} \quad S_{Risk}^i > \delta
\end{equation}
Where $N$ is the total number of scenes sampled, $S_{Risk}^i$ is the risk across the $i^{th}$ sampled scene, and $\delta$ is the risk threshold computed across the calibration set. 

% \textit{2) Diversity ($D$)} is a measure widely used to evaluate the tradeoff between exploration and exploitation~\cite{jerebic2021novel}. We measure diversity using the number of clusters and the quality of the cluster population as shown in \cref{eqn:diverse}. The cluster quality is measured as the average $S_{Risk}$ of the cluster population.

\textbf{2) Diversity ($D$)}: We measure diversity using two cluster-based quantities. (1) the number of optimal clusters that can be generated from the $N$ sampled scenes, as measured using silhouette score~\cite{rousseeuw1987silhouettes}. (2) the variance of risk across each scene across all the cluster. These quantities are combined into computing the diversity score as follows. 

% cluster quality is measured as the variance across the average $S_{Risk}$ of the different clusters.
\begin{equation}
\small
\label{eqn:diverse}
    % Diversity = \sum_{i=1}^{T_C} \left(\frac{1}{P^i}\sum_{j=1}^{P^i} S_{Risk} \right)
    Diversity = \sigma^2\{\frac{1}{len(\mathcal{C})}(\sum_{i=1}^{len(\mathcal{C})} S_{Risk}^i)|\forall \mathcal{C} \in N\}
\end{equation}    
    % \sigma^2\{\left(\frac{1}{P^i}\sum_{j=1}^{P^i} S_{Risk} \right) \quad | \quad \forall i \in \mathcal{C}\}   

Where $\mathcal{C}$ is a cluster of scenes generated on the scene variables. $N$ is the number of scenes sampled. $S_{Risk}^i$ is the risk of the $i^{th}$ scene in a cluster. To cluster the sampled scenes, we perform kmeans clustering~\cite{wagstaff2001constrained} on the scene variables. We then use the silhouette score~\cite{rousseeuw1987silhouettes} as the metric to select the optimal number of clusters. 

% That is, we choose the number of clusters that had the highest silhouette score.

\textbf{3) Search Time}: The overall time taken by the sampler to sample $N$ scenes and execute them in the simulator.

\input{results/comparison-table2}

\subsection{Results}
\label{sec:results}
To demonstrate our approach, we tasked the \ac{av} navigate different simulation scenes generated by the samplers. During these scenes, the \ac{ood} detector measures the martingale score, and the risk estimator estimates the collision rate $\lambda$ once every inference cycle. In these experiments, the simulation operates at a fixed rate of $20$ Frame Per Seconds. Also, to compare our samplers against the baselines, we executed each sampler for $250$ iterations. We started the samplers at the same initial condition with time-of-day = $45$ (noon) and a value of zero for the other variables. Also, instead of starting the \ac{gbo} sampler from scratch, we use the results from the random sampler to provide it a ``warm start". Further, for controlling the exploration vs. exploitation tradeoff, we empirically selected the following parameters. (1) Number of neighbors $K$ = 6, and neighborhood threshold $\tau$ = 10 for the \ac{rns} sampler, and (2) $\beta$ = 30 for the \ac{ucb} function of the \ac{gbo} sampler. 

\cref{fig:sampler_3d} shows the qualitative comparison of the scenes sampled by the samplers. As seen, the random and Halton samplers explore the search space, but they cannot exploit it because of their passive search strategy. On the other hand, the grid sampler exploits every point in the grid, but its exploration is limited.  In comparison, the \ac{rns} and \ac{gbo} samplers both explored and exploited the search space. 

% Further, we also compared the samplers using the comparison metrics.  


\textbf{Total Risk Scenes}: The total risk scenes generated by different samplers are shown in \cref{Table:comparison}. As seen, the random, Halton, and grid samplers sampled $66$\%, $71$\%, and $56$\% of high-risk scenes, respectively. In comparison, the \ac{rns} sampler sampled 83\% and \ac{gbo} sampled 92\% high-risk scenes among the $250$ scenes that were sampled. Also, \cref{fig:infractions} illustrates the number of \ac{ood} scenes and scenes with infractions that were generated by the samplers in $250$ iterations. As seen, the \ac{gbo} and the \ac{rns} samplers generated higher \ac{ood} scenes as compared to the baselines. Also, the \ac{rns} sampler had higher scenes with infractions followed by \ac{gbo} and Halton samplers.

\input{results/infractions}

\input{results/initial-conditions}


For further comparison, we start the simulator at $5$ different initial conditions varying the time-of-day (T), precipitation (P), and cloudiness (C) as illustrated in \cref{fig:initial}. The initial conditions are. (1) T = 0 (dawn), (2) T = 45 (noon), (3) T = 90 (dusk), (4) T = 45 (noon), P = 50\%, C = 50\%, and (5) T = 45, P = 0\%, C = 50\%, and the other variables were set to zero. Each sampler was executed for $50$ iterations from these initial conditions. As seen, the \ac{rns} and \ac{gbo} samplers generated high-risk scenes across the different starts as compared to the baselines. Among the baselines, the grid search generated higher high-risk scenes than the other two samplers. To note, the variable selection of the Halton sampler was not affected by the change in the starting conditions. 

\textbf{Diversity}: To compute diversity, we 
extract the clusters by applying kmeans clustering analysis along with silhouette score. As seen in \cref{Table:comparison}, the scenes generated by the \ac{rns} and \ac{gbo} samplers could be clustered into $6$ and $4$ clusters. Whereas the scenes generated by the Halton, grid, and random samplers could only be clustered in $2$, $2$, and $3$ clusters, respectively. We used these clusters to compute the diversity score in \cref{eqn:diverse}. As seen, the \ac{gbo} and \ac{rns} samplers had a higher diversity score of $0.63$ and $0.19$ as compared to the Halton, random, and grid samplers, which had scores of $0.07$, $0.02$, and $0.13$, respectively. The \ac{gbo} and \ac{rns} samplers had higher diversity because they had better exploration vs. exploitation trade-offs with a higher number of clusters from regions of the search space with higher $S_{Risk}$.


% despite having a lower number of clusters than the \ac{rns} sampler. This is because \ac{gbo} sampled clusters belonged to regions of the search space that had higher $S_{Risk}$. This is evident from \cref{fig:cluster}, which reports the cluster wise $S_{Risk}$ of all the samplers. In comparison, the baselines had a lower diversity score. 

% For this, we computed the variance across the average $S_{Risk}$ of the different clusters.

% It can be seen that the other samplers missed the critical high-risk areas that the \ac{gbo} sampler could identify. 

\begin{figure}[!t]
\input{results/cluster}
 \vspace{-0.1cm} 
 \input{results/cluster1}
\footnotesize
\centering
\setlength{\abovecaptionskip}{2pt}
\caption{The variance of $S_{Risk}$ across scene clusters generated by different samplers. Our samplers generate higher clusters with a high variance of $S_{Risk}$. Y-axis shows the number of clusters, and the Y-axis shows the $S_{Risk}$ score.}
\label{fig:cluster}
\vspace{-0.1in}
\end{figure}

\input{results/samples}

\textbf{Search Times}: We report the search times of the samplers in \cref{Table:comparison}. As seen, the random, Halton, grid, and \ac{rns} samplers have comparable search times of $323$, $315$, $309$, and $332$ minutes, respectively. However, the \ac{gbo} sampler required the highest search time of $897$ minutes because of its scalability issue discussed in \cref{sec:gbo_sampler}. In addition, \cref{fig:samplers_perf} reports the number of scenes generated by these samplers in $60$ minutes. The \ac{rns} sampler and the baselines roughly sampled $40$ scenes in $60$ minutes. But, the \ac{gbo} sampler only sampled $19$ scenes. 

% in the allotted time. 



% The \ac{gbo} sampler suffers from the scalability issue discussed earlier. This causes the \ac{gbo} sampler to sample only $19$ scenes, while all the other samplers roughly sample $40$ scenes in the allotted time. 

\textbf{Summary}: The key takeaways from the experiments are. \underline{First}, we observe that in general, the \ac{rns} and \ac{gbo} samplers outperform the baselines by generating a higher percentage of high-risk scenes (first objective). \underline{Second}, we observe that the scene generated by the \ac{rns} and \ac{gbo} samplers could be clustered into more clusters with higher variance compared to the baselines (second objective). \underline{Third}, the \ac{gbo} sampler is the most effective in generating high-risk scenes, and its informed exploration results in highly diverse search. But, the use of \ac{gp} model increases the search time. In comparison, the \ac{rns} sampler is efficient and requires lower search times to generate high-risk scenes. 



% history of the search space is available. (b) there is no time budget for the search. However, the \ac{rns} sampler is efficient with lower search times compared to the \ac{gbo} sampler. 


% and it can be used when (a) some history of the search space is available. (b) there is no time budget for the search process. However, when no past search information is available, the \ac{rns} sampler can be used.  









==> Version1/individual-sections/problem-statement.tex <==
\section{Problem Formulation}
\label{sec:ps}
\subsection
We use an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to set up the problem. The \ac{av} is tasked to navigate an urban town with complex traffic scenarios including changing weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. The \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation. Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.

% Given this simulator, the \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation.  

The \ac{lec} is trained on a training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes. A scene $s$ is a short time-series trajectory (typically 30 seconds to 60 seconds) of the \ac{av}'s journey in the environment. It can be represented as a sequence of entries at each time step, where each entry is defined by different environmental variables ($e_v$) and agent variables $a_v$. The environment can be captured using different structural variables (e.g., road segments, waypoints, road geometry) and temporal variables (e.g., weather, time-of-day, traffic). The agent variables can be operating modes, sensor faults, failure modes, etc. These scene variables $s_v$ are mostly defined by a distribution $\mathcal{P} \in [lower,upper]$. The combination of these scene variables form a search space $\mathcal{D}$, which can be sampled to generate different scenes. However, each of these variables may have different constraints $C$ as discussed earlier. 
For example, in the CARLA case study, the CARLA map defines the list of adjacent road segments, which forms the structural constraints. Similarly, there may be constraints on the rate of change in the values of the environmental variables. For example, the precipitation levels cannot drastically change from 10\% to 90\%, it can only gradually increase at a defined rate. Also, each scene is associated with a risk score $R_S$ estimated by the risk estimator. 


Given this setup, the problem we study in this work is to design sampling approaches that can find the following.  

\begin{enumerate}
    \item Given the scene variables $s_v$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate a scene $s_i$ that has a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
    
    \item Given the scene variables $s_v$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate cluster of similar scenes $C_s$ that have a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
\end{enumerate}
    

% \begin{problem}
% \label{prob:high-risk scene}
% Given the scene variables $S_V$ and the search space $\mathcal{D}$, generate a scene $s_i$ that has a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
% \end{problem}

% \begin{problem}
% \label{prob:cluster scene}
% Given the scene variables $S_V$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate cluster of similar scenes $C_s$  that have a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
% \end{problem}


% With this set up, we can define the problems we study as follows:

% \ac{lec} is trained on sensor data in the training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes.

==> Version1/individual-sections/problem-statement1.tex <==
\section{Problem Formulation}
\label{sec:ps}
We consider the autonomous \ac{cps} to be operating in an environment, characterized by two sets of variables $\mathbb{E}: x \rightarrow \Re^{+}$ and $\mathbb{S}: y \rightarrow \Re^{+} \times \Re^{+}$. The $\mathbb{E}$ are the environmental variables like rain, traffic density, time-of-the-day. The $\mathbb{S}$ are structural variables related to roadway features and are characterized by waypoints $w$ denoted by a two dimensional matrix of latitude and longitude. Each waypoint can be mapped to a road segment and provides the features of the road: gradient, elevation, number of lanes. In addition, we consider the set of faults in the system sensors and actuators $F: x \rightarrow {0,1}$. For a particular operating environment, there can be several environment variables $e \in \mathbb{E}$, several possible waypoints $w \in \mathbb{S}$, and several sensors in the system that can fail and impact the system's safety, $f \in \mathbb{F}$. The \ac{cps} is trained through a collection of scenes $\mathcal{T}$, where each scene $s$ is an ordered sequence of $K$ sampled observations (samples for short) $< s_i=(\mathbb{E}_i, \mathbb{S}_i, \mathbb{F}_i) >_{i=1}^{K}$. These three variables are collectively called the scene variables $s_V$ in this work. Given each scene $s_i$, we can associate the likelihood of hazard rate ($\lambda$) for every hazard that is identified for the system. To remind, the system can have a collection of hazards $\{H_1,H_2,\cdots,H_n\}$ stemming from its components (e.g., software, hardware) or its operating conditions. Each identified hazard will have an associated hazard rate estimated using the dynamic assurance routines ($DA: s \rightarrow \lambda$) introduced in \cref{sec:risk_estimation}. The hazard rate can be used to compute the likelihood of the hazard occurrence in a given time unit $1-e^{-\lambda \cdot t}$. Where $\lambda$ is the estimated hazard rate, and $t$ is the operation time. The estimated likelihood of hazard for different hazard conditions put together constitutes the system's operational risk $S_{Risk}$. 

\input{results/constraints}

\begin{figure*}[!ht]
\centering
 \includegraphics[width=0.92\textwidth]{figures/workflow10.pdf}
 \caption{Overview of the proposed approach, which includes a \acl{sdl} integrated with two samplers and a scoring function for generating high-risk scenes. The samplers perform active sampling using the feedback loop (red dotted line). Our approach is designed for the testing phase of \ac{cps}.}
 \label{fig:workflow}
% \vspace{-0.1in}
\end{figure*}


% \footnote{It is common to use latitude and longitude as the waypoint}.

Also, given a sequence of samples in the scenes, physical constraints govern the temporal evolution of the sampled values. For example, a constraint on an environmental variable $e \in \mathbb{E}$ governs that $|s_i^e-s_{i+1}^e| \leq \alpha_e \in \Re^+$. Similarly, the waypoints across a scene are governed by routability property. To explain this, we use the sampling constraints $\mathcal{SC}$ (See \cref{Table:constraints}) that we applied for an \ac{av} case study that will be discussed in \cref{sec:casestudy}. The road segment is governed by the constraint that the distance between two selected waypoints cannot be greater than $10$ meters. This constraint regulates that the road segment is orderly selected. The environmental variables have constraints on how much their values change between consecutive scenes. The traffic density has constraints on its value and is also dependent on the type of road segment (e.g., crossroads, intersections). Also, we did not place any constraints on the fault variables. Now, given this setup, we want to address the following problem. 

% Without these constraints, we found the sampled scene sequence was unrealistic. Two such scenes were  

% the trained \ac{cps} and its operating conditions, we want to address the following problems. 

\begin{problem}
\label{prob:high-risk scene}
Given a threshold $\delta$ (computed across the previously observed train scenes), sample $N$ scenes that maximizes the risk $\max(sum(S_{Risk} - \delta))$. In addition we want to ensure that the scene variables are diverse. We call a scene with $S_{Risk} - \delta > 0$  as a high risk scene.

% diversity across the clusters is maximized 


% $\max(\sigma^2\{\frac{1}{len(\mathcal{C})}\sum_{i=1}^{len(\mathcal{C})} (S_{Risk}^i-\delta) |  \forall \mathcal{C} \in N\})$ 
\end{problem} %\textcolor{red}{This is not correct. The diversity is on the features of the scenes and should not have anything to do with the $S_{Risk}$. Perhaps just explain this is in simple words if you cannot explain in mathematics}


% maximizes the diversity $\max(\sigma^2(S_{Risk} - \delta))$. 

% dissimilarity of the $N$ Scenes that have been sampled.
%Find scenes that have $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from previously observed scenes. 


% \begin{problem}
% \label{prob:cluster scene}
% Find clusters of similar scenes that have $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from previously observed scenes 
% \end{problem}

% Where $\delta$ is the risk threshold computed across the previously observed train scenes. A scene with $S_{Risk} - \delta > 0$ is termed to as high-risk scene in this work. Now, our goal in this work is to design a ``\textit{Sampler}" which can address the problem. The problem can be expressed as two objectives of the sampler. The first objective of the sampler is to sample a higher number of high-risk scenes. The second objective of the sampler is to sample a higher number of scenes clusters, such that the variance of risk across the clusters is high. While the first objective measures the sampler's capability of finding the region of the search space with high-risk scenes, the second measures the sampler's diversity,which is a measure of the sampler's exploration vs. exploitation trade-off. High diversity is desirable to better cover the search space~\cite{jerebic2021novel}. We measure diversity in terms of a quantitative metric (measured using the number of the cluster) and a qualitative metric (measured using the variance of risk across clusters). 

% Recall, our goal is to design a %``\textit{Sampler}" which can address the problem. 
%The problem can be expressed as two objectives. The first objective is to sample a large number of high-risk scenes. The second objective is to ensure diversity across the sampled scenes. 
%higher number of scenes clusters, such that the variance of risk across the clusters is high.
While the first objective measures the sampler's capability of finding the region of the search space with high-risk scenes, the second measures the sampler's diversity, which represents the sampler's capability to balance between exploration vs. exploitation. A sampler with high diversity is desirable for better coverage of the search space~\cite{jerebic2021novel}. We measure diversity in terms of a quantitative metric (measured using the number of the optimal clusters, as measured using silhouette score~\cite{rousseeuw1987silhouettes}) and a qualitative metric (measured using the variance of risk across each scene across all clusters). 




% First, sample a higher number of high-risk scenes. This measures the sampler's capability of finding the region of the search space with high-risk scenes. Second, sample a higher number of scenes in clusters, such that the variance of risk across the clusters is high. This measures the sampler's diversity, which is a measure of the sampler's exploration vs. exploitation trade-off. High diversity is desirable to better cover the search space~\cite{jerebic2021novel}. We measure diversity in terms of a quantitative metric (measured using the number of the cluster) and a qualitative metric (measured using the variance of risk across clusters). 




% Diversity is a measure used to evaluate the exploration vs. exploitation trade-off, which is a desirable property to better cover the search space~\cite{jerebic2021novel}. So, our objective is to maximize the diversity. 

 
% to have higher number of clusters and higher variance

% Second, sample scenes in clusters such that the variance of risk across the clusters is maximized. We use variance as the measure of the sampler's diversity. The diversity is a measure widely used to evaluate the exploration vs. exploitation trade-off~\cite{jerebic2021novel}. In our setup, it is measured as the variance of $S_{Risk}$ across the clusters that are generated from the $N$ sampled scenes. So, higher the variance, better is the exploration vs. exploitation strategy. 

% Now, our goal in this work is to design a ``\textit{Sampler}" which can address the problem. 
% Addressing the problem is relevant for the uses cases briefly introduced earlier. That is, addressing the first part of the problem will generate the high-risk scenes that can be used for testing and validating the system. Addressing the second part will generate clusters of similar high-risk scenes which can be used for continually improving models.  

% We refer to high-risk scenes when we use the term ($S_{Risk} - \delta$)

% To explain these problems, we setup an \ac{av} case study in CARLA simulator~\cite{dosovitskiy2017carla}. In this example, an \ac{av} is tasked to navigate an urban town with complex traffic conditions, adverse weather conditions (e.g., high lighting level, high precipitation), and sensor faults (e.g., camera failure). These simulation parameters are the scene variables, which we sample based on the sampling constraints in \cref{Table:constraints} to generate scenes with varying operating conditions. Also, to evaluate the \ac{av}'s performance, we leverage the infraction metrics returned by the CARLA autonomous driving challenge ~\cite{carla-challenge}. Specifically, we use the system infractions like running a red light, running a stop sign, route deviation, off-road driving, etc. Now, given this simulation setup, the goal of the \ac{av} is to navigate the different scenes without collisions. For this, the \ac{av} is augmented with safety components anomaly detectors, an \ac{ood} detector and a risk estimator~\cite{hartsell2021resonate} for dynamic assurance routines. These components together estimate the \ac{av}'s hazard rate and its operational risk in a given scene ($DA: S \rightarrow S_{Risk}$). With this setup, we train an \ac{lec} controller to operate the \ac{av} and calibrate the safety components with several train and calibration scenes which we will discuss in \cref{sec:evaluation}. Now, given the trained \ac{av}, our goal is to design a sampler for sampling high-risk test cases for the \ac{av}.

% find test scenes that are of high-risk to the \ac{av}. For this, our goal is to design a sampler that can address the two problems discussed above.


==> Version1/individual-sections/problem-statement2.tex <==
\section{Problem Formulation}
\label{sec:ps}
\textbf{Problem Setup}: To set up the problem, consider an autonomous \ac{cps} operating in a simulator. This system uses an \ac{lec} for navigation, and it is augmented with safety components such as anomaly detector, \ac{ood} detector, and risk estimators for dynamic assurance and estimating the system's operational risk. These components are usually trained and calibrated on sensor data (e.g., camera images, radar signals) collected from a training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes. 

A scene $s$ is a short sequence of sampled observations. Each sample is an indexed entry from the scene and provides a value to three class of variables 

(typically 30 seconds to 60 seconds) of the system's journey in the environment. It can be represented as a time-stamped sequence of entries, where each entry is defined by different environmental variables ($e_v$) and agent variables $a_v$. The environment can be captured using different structural variables (e.g., road segments, waypoints, road geometry) and temporal variables (e.g., weather, time-of-day, traffic). The agent variables can be operating modes, sensor faults, failure modes, etc. These scene variables $s_v$ are mostly defined by a distribution $\mathcal{P} \in [lower,upper]$. 

The combination of these scene variables forms a search space $\mathcal{D}$, which can be sampled to generate different scenes. However, these variables may have constraints that need to be included during sampling. For example, the structural variables such as road segments and waypoints may have sequential ordering constraints defined by the simulator's map. Similarly, temporal variables like the weather parameters (e.g., lighting) may have constraints on the rate at which their values change. In addition, each scene is associated with a risk score $S_{Risk}$ estimated by the risk estimator. Now, given the trained system with the calibrated risk estimator, we want to generate scenes in which the system is susceptible to failure. For this, our goal is to design a sampler that can address the following problems.    

% in the CARLA case study, the CARLA map defines the list of adjacent road segments, which forms the structural constraints. Similarly, there may be constraints on the rate of change in the values of the environmental variables. For example, the precipitation levels cannot drastically change from 10\% to 90\%, it can only gradually increase at a defined rate. Also, each scene is associated with a risk score $S_{Risk}$ estimated by the risk estimator. Given this set up, the goal is to test the \ac{cps} across scenes where it fails. For this, the goal of this work is to design a sampler that can address the following problems.  
    
\begin{problem}[Sample High-Risk Scene]
\label{prob:high-risk scene}
Given the scene variables $S_V$, the search space $\mathcal{D}$, and the sampling constraints, sample scenes $s_i$ that have risk $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from the previously observed scenes. 
\end{problem}

\begin{problem}[Sample Cluster of High-Risk Scenes]
\label{prob:cluster scene}
Given the scene variables $S_V$, the search space $\mathcal{D}$, and the sampling constraints, sample clusters of similar scenes $C_s$ that have risk $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from the previously observed scenes 
\end{problem}

\textbf{Case Study}: We consider an \ac{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to explain these problems. In this example, an \ac{av} is tasked to navigate an urban town with complex traffic conditions, adverse weather conditions (e.g., high lighting level, high precipitation), and sensor faults (e.g., camera failure). These simulation parameters are the scene variables, which we sample to generate scenes with varying operating conditions. Also, to evaluate the \ac{av}'s performance, we leverage the infraction metrics returned by the CARLA autonomous driving challenge ~\cite{carla-challenge}. Specifically, we use the system infractions like running a red light, running a stop sign, route deviation, off-road driving, etc. Now, given this simulation setup, the goal of the \ac{av} is to navigate the different scenes without collisions. For this, the \ac{av} is augmented with several anomaly detectors, an \ac{ood} detector and a risk estimator~\cite{hartsell2021resonate} to estimate the \ac{av}'s risk of collision across an operating scene. The \ac{lec} controller is trained, and the risk estimator is calibrated using several train and calibration scenes. The specifics of the \ac{av} setup and training are discussed in \cref{sec:evaluation}. Now, given the trained \ac{av}, our goal is to find test scenes that are of high-risk to the \ac{av}. For this, our goal is to design a sampler that can address the two problems discussed above.




% Now, given the trained \ac{av}, we want to test it across different scenes where it is susceptible to failure. For this, our goal is to design a sampling approach that can sample. (1) scenes $s_i$ with different operating conditions and camera faults that has a risk greater than the risk across the training scenes. and (2) a cluster of scenes $C_s$ with similar operating conditions and camera faults that have a risk greater than the risk across the training scenes. 

% To address these problems, we design two sequential sampling approaches that considers the sampling constraints and provides an explicit control over the exploration and exploitation of the search space. The sampling approaches are discussed in the following section. 

% To explain these problems, we consider an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla}. We rely on the CARLA autonomous driving challenge ~\cite{carla-challenge} setup that allows simulating complex traffic scenes and it also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. This set up allows us to generate different traffic scenes by varying weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. In addition, it also allows us to inject different faults (e.g., camera occlusion, camera blur) into the \ac{av}'s sensors.  

% The \ac{av} in this set up is driven by a navigation \ac{lec} controller and it has an \ac{ood} detector and a \ac{resonate} risk estimator~\cite{hartsell2021resonate} as the safety components for runtime monitoring. The controller and the components are trained and calibrated using a set of scenes $\mathcal{T}$ generated by randomly varying the weather, traffic and pedestrian density, and road segments. Each of these scenes has an associated risk $R$ of \ac{av}'s collision as estimated by the risk estimator. Now, given simulator set up and the \ac{av}, the goal is to design a sampler that can find. (1) a single scene $s_i$ with different operating conditions and camera faults that has a risk greater than the risk across the training scenes, and (2) a cluster of scenes $C_s$ with similar operating conditions and camera faults that has a risk greater than the risk across the training scenes.     


% Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.

% \subsection{Case Study}
% We use an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to set up the problem. The \ac{av} is tasked to navigate an urban town with complex traffic scenarios including changing weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. The \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation. Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.



==> Version1/individual-sections/related-works.tex <==
\section{Related Work}
\label{sec:rw}
% The task of generating high-risk or safety critical scenes has been addressed in the literature using. 1) sampling-based approaches, 2) 

% can be broadly classified into three categories. 1) sampling

% The generation of high-risk or safety-critical scenes in simulation has gained significant interest in recent years. 
Tools like Dakota~\cite{dalbey2021dakota} with sampling approaches like incremental sampling, importance sampling, and adaptive sampling have been long available for uncertainty quantification in engineering design. Such samplers have recently gained interest for sampling simulation-based scenes in the \ac{av} domain. Several domain-specific \acp{sdl} like Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} have been designed for specifying scenarios of complex traffic conditions and operating conditions to identify edge cases and counterexamples that affect the system's safety. These languages are mostly designed for the \ac{av} domain to work with the CARLA simulator~\cite{dosovitskiy2017carla}. These languages are equipped with probabilistic samplers that sample scenes across the entire search space formed by the combination of scene variables. For example, Grid search is a popular passive sampler, which takes a single risky scene as the starting condition and generates similar risky scenes around it. However, manual tuning makes the grid sampler labor-intensive and time consuming. For accelerating the search process, an alternate approach~\cite{zhao2017accelerated} uses importance sampling to identify important scene variables and sample scenes using them. Worst-Case Scenario Evaluation~\cite{ma1999worst} is another approach that uses model-based optimization to identify the weakness of the system and uses this information to generate worst-case disturbances. VERIFAI~\cite{dreossi2019verifai} software toolkit has several passive samplers like random search, Halton search~\cite{halton1960efficiency}, and active samplers like cross-entropy optimization and \acl{bo}. But, these samplers cannot control the exploration vs. exploitation trade-off during sampling. 
This is addressed by a multi-armed bandit sampler that balances the two strategies~\cite{viswanadha2021parallel}. 

% As discussed by Ding, Wenhao, \emph{et al.}~\cite{ding2020learning}, g

% There have also been other approaches. Grid search is another popular passive sampler, which takes a single risky scene as the starting condition and generates similar risky scenes around it. However, manual tuning makes the grid sampler labor-intensive and time consuming. For accelerating the search process, an alternate approach~\cite{zhao2017accelerated} uses importance sampling to identify important scene variables and sample scenes using them. Worst-Case Scenario Evaluation~\cite{ma1999worst} is another approach that uses model-based optimization to identify the weakness of the system and uses this information to generate worst-case disturbances. 


% There have also been other approaches. Grid search is a popular passive sampling approach used in industry. Here, a previously identified risky scene is used as the initial condition, and the grid around is searched to sample similar risky scenes. Manual tuning makes the grid sampler labor-intensive and time consuming. For accelerating the search process, an alternate approach~\cite{zhao2017accelerated} uses importance sampling to identify important scene variables and sample scenes using them. Worst-Case Scenario Evaluation~\cite{ma1999worst} is another approach that uses model-based optimization to identify the weakness of the system and uses this information to generate worst-case disturbances. 

Also, recently, there has been growing interests in using deep generative models for generating risky scenes~\cite{ding2018new,vardhan2021rare,o2018scalable,ding2020learning}. In this approach, scenes are randomly sampled from a learned distribution instead of sampling from the entire search space. Ding, Wenhao, \emph{et al.}~\cite{ding2020learning} use an autoregressive model to factorize the scene variables into conditional probability distributions, which are then sampled to generate risky traffic scenes. In a prior work~\cite{ding2018new}, they have also used a \acl{vae} to project high-dimensional traffic information into a lower-dimensional latent space, which is sampled to generate critical traffic scenes. Vardhan \emph{et al.}~\cite{vardhan2021rare} use a Gaussian Mixture Model to find the corner case scenes in the training set that is not well learned by the system. Another approach~\cite{o2018scalable} uses an ensemble of generative adversarial imitation learning to perform adaptive importance-sampling to learn rare events from an underlying data distribution. 



% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 















% The generation of scenes covering the entire range of expected environmental conditions has become an important study for testing and validating autonomous \ac{cps}. Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} are well-known domain-specific \acp{sdl} used for scene generation. These languages have been equipped with probabilistic samplers to sample different values for the scene variables. Grid search is a brute force approach widely adopted in the industry. In this approach, a previously identified risky scene is used as the initial condition, and the grid around it is searched to sample risky scenes~\cite{ding2020learning}. This approach requires prior information of the risk scenes and can be labor-intensive. Instead of starting from manually identified risk scenes, an importance sampling approach for accelerated identification of high-risk scenes is proposed ~\cite{ding2020learning}. VERIFAI~\cite{dreossi2019verifai} provides several sampling approaches like random search, Halton search, cross-entropy optimization, and \acl{bo}, which is integrated with Scenic~\cite{fremont2019scenic} to generate scenes with counterexamples. Also, recently, the scene sampling process is formulated as a multi-armed bandit problem, which seeks to balance between exploration vs. exploitation ~\cite{viswanadha2021parallel,viswanadha2021addressing}.

% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 

==> Version1/individual-sections/rw.tex <==
\section{Related Work}
\label{sec:rw}
% The task of generating high-risk or safety critical scenes has been addressed in the literature using. 1) sampling-based approaches, 2) 

% can be broadly classified into three categories. 1) sampling

% The generation of high-risk or safety-critical scenes in simulation has gained significant interest in recent years. 
Tools like Dakota~\cite{dalbey2021dakota} with sampling approaches like incremental sampling, importance sampling, and adaptive sampling have been long available for uncertainty quantification in engineering design. Such samplers have recently gained interest for sampling simulation-based scenes in the \ac{av} domain. Several domain-specific \acp{sdl} like Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} have been designed for specifying scenarios of complex traffic conditions and operating conditions to identify edge cases and counterexamples that affect the system's safety. These languages are mostly designed for the \ac{av} domain to work with the CARLA simulator~\cite{dosovitskiy2017carla}. These languages are equipped with probabilistic samplers to sample values for scene variables from their distribution ranges, thus generating different scenes. For example, the Scenic language is integrated with the VERIFAI~\cite{dreossi2019verifai} software toolkit that has several passive samplers like random search, Halton search~\cite{halton1960efficiency}, and simulated annealing, which do not use the previous results to perform an informed sampling. Additionally, they include active samplers like cross-entropy optimization and \acl{bo}, which use a feedback loop of previous results in the sampling process. These samplers cannot control the exploration vs. exploitation tradeoff during sampling. To address this, a multi-armed bandit sampler that balances the two strategies is proposed~\cite{viswanadha2021parallel}. 

% As discussed by Ding, Wenhao, \emph{et al.}~\cite{ding2020learning}, g

There have also been other approaches. Grid search is a popular passive sampling approach used in industry. Here, a previously identified risky scene is used as the initial condition, and the grid around is searched to sample similar risky scenes. Manual tuning makes the grid sampler labor-intensive and time consuming. For accelerating the search process, an alternate approach~\cite{zhao2017accelerated} uses importance sampling to identify important scene variables and sample scenes using them. Worst-Case Scenario Evaluation~\cite{ma1999worst} is another approach that uses model-based optimization to identify the weakness of the system and uses this information to generate worst-case disturbances. 

In addition to the conventional samplers, there have recently been growing interests in using deep generative models for generating risky scenes~\cite{ding2018new,vardhan2021rare,o2018scalable,ding2020learning}. These approaches sample scenes from a learned distribution instead of sampling from the entire search space. Ding, Wenhao,\emph{et al.}~\cite{ding2020learning} use an autoregressive model to factorize the scene variables into conditional probability distributions, which are then sampled based on conditional dependence to generate risky traffic scenes. In a prior work~\cite{ding2018new}, they have also used a \acl{vae} to project high-dimensional traffic information into a lower-dimensional latent space, which is sampled to generate critical traffic scenes. Vardhan \emph{et al.}~\cite{vardhan2021rare} use a Gaussian Mixture Model to find the corner case scenes in the training set that is not well learned by the system. Another approach~\cite{o2018scalable} uses an ensemble of generative adversarial imitation learning to perform adaptive importance-sampling to learn rare events from an underlying data distribution. 



% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 















% The generation of scenes covering the entire range of expected environmental conditions has become an important study for testing and validating autonomous \ac{cps}. Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} are well-known domain-specific \acp{sdl} used for scene generation. These languages have been equipped with probabilistic samplers to sample different values for the scene variables. Grid search is a brute force approach widely adopted in the industry. In this approach, a previously identified risky scene is used as the initial condition, and the grid around it is searched to sample risky scenes~\cite{ding2020learning}. This approach requires prior information of the risk scenes and can be labor-intensive. Instead of starting from manually identified risk scenes, an importance sampling approach for accelerated identification of high-risk scenes is proposed ~\cite{ding2020learning}. VERIFAI~\cite{dreossi2019verifai} provides several sampling approaches like random search, Halton search, cross-entropy optimization, and \acl{bo}, which is integrated with Scenic~\cite{fremont2019scenic} to generate scenes with counterexamples. Also, recently, the scene sampling process is formulated as a multi-armed bandit problem, which seeks to balance between exploration vs. exploitation ~\cite{viswanadha2021parallel,viswanadha2021addressing}.

% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 

==> Version1/paper.tex <==
\section{Introduction}
The widespread use of autonomous \acp{cps}\footnote{CPS with \ac{lec}} has often required them to operate under uncertainties like sensor degradation and shifts in the operating conditions~\cite{schwalbe2020survey}, which increase its operational risk. Design-time Assurance Cases~\cite{bishop2000methodology} and risk assessment are used to argue the system's safety at runtime. However, design-time information is inadequate for runtime estimations~\cite{denney2015dynamic} and a dynamic assurance approach is needed to handle the dynamically changing operating conditions in which the system operates. Dynamic Assurance requires designing runtime monitors like \ac{ood} detectors~\cite{sundar2020out} and risk estimators~\cite{hartsell2021resonate} for identifying the distribution shift in the operating condition and estimating the system's risk of failure. Designing these components often requires labeled data from scenes of failure conditions and corner cases in which the system fails. These scenes are commonly referred to as worst case scenarios~\cite{worstcaserl} or safety-critical scenarios~\cite{ding2020learning}; in this paper, we refer to them as high-risk scenes.


Similar to the \ac{ood} problem~\cite{cai2020real,sundar2020out,schwalbe2020survey}, often the data related to risky scenarios is under-represented in the training sets~\cite{khan2019striking}, leading to a data imbalance problem. If we can generate these under-represented events, they can be used to retrain the models to improve their accuracy~\cite{fremont2019scenic}. Further, such new scenes can be used for updating the machine learning components. However, collecting real-world data of such high-risk scenes can be expensive and slow in real-world conditions. There has been a growing interest in using synthetic data from simulators to address this problem~\cite{zhao2017accelerated,ma1999worst,dreossi2019verifai,viswanadha2021parallel}. For example, domain-specific \ac{sdl} like Scenic \cite{fremont2019scenic}, and MSDL \cite{msdl} provide probabilistic sampling capability integrated with CARLA \cite{dosovitskiy2017carla} to generate meaningful high-risk scenes. In addition, tools like Dakota~\cite{dalbey2021dakota} provide efficient sampling approaches like incremental sampling, importance sampling, and adaptive sampling and have been used for uncertainty quantification in engineering design.

Despite their success in generating high-risk scenes, we point to several limitations. First, the existing approaches perform \textit{passive sampling}, which does not use feedback from the previous results in the sampling process. Second, the scene variables being sampled typically have \textit{sampling constraints} and \textit{co-relations} that need to be considered. For example, the environmental properties of a scene (e.g., precipitation) may have physical constraints on their values that govern its temporal evolution. Applying these constraints is necessary for generating meaningful scenes~\cite{fremont2019scenic}. But the existing approaches do not include these sampling constraints. Third, conventional samplers do not balance the \textit{exploration vs. exploitation trade-off}. For example, Random search and Halton search prioritize coverage of the search space through uniform exploration. Alternately, Grid search aims for exhaustively covering a given grid, so they only exploit. However, balancing these strategies can result in higher coverage diversity, which is often measured using clustering properties like the number of clusters and cluster population~\cite{jerebic2021novel}. 


% For example, random search can only explore the search space, and grid search can only exploit a given grid. However, as discussed by Jerebic, Jernej \emph{et al.}~\cite{jerebic2021novel}, balancing these strategies can better cover the search space. The coverage diversity can be measured using clustering properties like the number of clusters and cluster population. 

We present a scene generation approach that has a domain-specific \ac{sdl} integrated with two sampling approaches for generating high-risk simulation scenes. The key contribution of our work are two sampling approaches called \ac{rns} and \ac{gbo}. These samplers perform active sampling by using feedback of previous simulation results in the sampling process. They also include sampling constraints that govern the evolution of scene variables. In addition, they provide explicit hyperparameters to control the tradeoff between exploration vs. exploitation of the search strategy, using a novel risk-based scoring function. We demonstrate our approach using an \ac{av} case study in the CARLA simulator \cite{dosovitskiy2017carla}. To evaluate our samplers, we compared them against the baselines of random search, grid search, and Halton sequence search~\cite{halton1960efficiency} in terms of the total risk scenes, diversity, and search time metrics. Our experimental evaluation shows that the \ac{rns} and \ac{gbo} outperform the baselines in terms of the total risk scenes and diversity metrics. Also, the \ac{rns} sampler had comparable search times to the baselines, but the \ac{gbo} sampler has a higher search time. The source code and the technical appendix are available online\footnote{\label{github}https://github.com/Shreyasramakrishna90/Risk-Aware-Scene-Generation}.

% \footnote{\label{github}\url{https://github.com/Shreyasramakrishna90/Risk-Aware-Scene-Generation}}.

\begin{figure}[t]
 \centering
 \includegraphics[width=\columnwidth]{figures/system-model3.pdf}
 \caption{System model of the \ac{av} designed for the CARLA challenge example. The \ac{av} is primarily driven by an \ac{lec}-based navigation controller, which is supervised by an AEBS for emergency braking. The \ac{lec} predicted control signals are sent to the \ac{av} operating in the simulator.} 
 \label{fig:sys-model}
\vspace{-0.1in}
\end{figure}

The outline of this paper is as follows. In \cref{sec:background}, we introduce the background on the typical design process and a dynamic assurance framework that we use. In \cref{sec:ps}, we describe the problem statement, followed by a description of our approach in \cref{sec:approach}. In \cref{sec:evaluation}, we implement and evaluate the samplers in the context of CARLA autonomous driving challenge~\cite{carla-challenge}. This setup requires an \ac{av} to navigate an urban town setting with complex traffic scenarios, adverse weather conditions, and sensor faults. The system model of the \ac{av} is shown in \cref{fig:sys-model}. Finally, we present related research in \cref{sec:rw} followed by conclusions in \cref{sec:conclusion}. 


\begin{figure*}[t]
 \centering
 \includegraphics[width=0.9\textwidth]{figures/btd.pdf}
 \caption{Bow-Tie Diagram for the \ac{av} case study adopted from our previous work~\cite{hartsell2021resonate}. Each block includes information about the event type and its description. The conditional probability and the threat $LUT$s are estimated from training data and discussed in \cref{sec:risk}.}
 \label{fig:btd}
\end{figure*}

==> individual-sections/problem-statement.tex <==
\section{Problem Formulation}
\label{sec:ps}
\subsection
We use an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to set up the problem. The \ac{av} is tasked to navigate an urban town with complex traffic scenarios including changing weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. The \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation. Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.

% Given this simulator, the \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation.  

The \ac{lec} is trained on a training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes. A scene $s$ is a short time-series trajectory (typically 30 seconds to 60 seconds) of the \ac{av}'s journey in the environment. It can be represented as a sequence of entries at each time step, where each entry is defined by different environmental variables ($e_v$) and agent variables $a_v$. The environment can be captured using different structural variables (e.g., road segments, waypoints, road geometry) and temporal variables (e.g., weather, time-of-day, traffic). The agent variables can be operating modes, sensor faults, failure modes, etc. These scene variables $s_v$ are mostly defined by a distribution $\mathcal{P} \in [lower,upper]$. The combination of these scene variables form a search space $\mathcal{D}$, which can be sampled to generate different scenes. However, each of these variables may have different constraints $C$ as discussed earlier. 
For example, in the CARLA case study, the CARLA map defines the list of adjacent road segments, which forms the structural constraints. Similarly, there may be constraints on the rate of change in the values of the environmental variables. For example, the precipitation levels cannot drastically change from 10\% to 90\%, it can only gradually increase at a defined rate. Also, each scene is associated with a risk score $R_S$ estimated by the risk estimator. 


Given this setup, the problem we study in this work is to design sampling approaches that can find the following.  

\begin{enumerate}
    \item Given the scene variables $s_v$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate a scene $s_i$ that has a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
    
    \item Given the scene variables $s_v$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate cluster of similar scenes $C_s$ that have a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
\end{enumerate}
    

% \begin{problem}
% \label{prob:high-risk scene}
% Given the scene variables $S_V$ and the search space $\mathcal{D}$, generate a scene $s_i$ that has a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
% \end{problem}

% \begin{problem}
% \label{prob:cluster scene}
% Given the scene variables $S_V$, the search space $\mathcal{D}$, and sampling constraints ($C$) generate cluster of similar scenes $C_s$  that have a risk score $R_S$ $\geq$ risk across the training scenes $R_T$. 
% \end{problem}


% With this set up, we can define the problems we study as follows:

% \ac{lec} is trained on sensor data in the training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes.

==> individual-sections/problem-statement2.tex <==
\section{Problem Formulation}
\label{sec:ps}
\textbf{Problem Setup}: To set up the problem, consider an autonomous \ac{cps} operating in a simulator. This system uses an \ac{lec} for navigation, and it is augmented with safety components such as anomaly detector, \ac{ood} detector, and risk estimators for dynamic assurance and estimating the system's operational risk. These components are usually trained and calibrated on sensor data (e.g., camera images, radar signals) collected from a training distribution $\mathcal{T}$, where $\mathcal{T}$ = \{$s_1,s_2, \dots,s_m$\} is a collection of scenes. 

A scene $s$ is a short sequence of sampled observations. Each sample is an indexed entry from the scene and provides a value to three class of variables 

(typically 30 seconds to 60 seconds) of the system's journey in the environment. It can be represented as a time-stamped sequence of entries, where each entry is defined by different environmental variables ($e_v$) and agent variables $a_v$. The environment can be captured using different structural variables (e.g., road segments, waypoints, road geometry) and temporal variables (e.g., weather, time-of-day, traffic). The agent variables can be operating modes, sensor faults, failure modes, etc. These scene variables $s_v$ are mostly defined by a distribution $\mathcal{P} \in [lower,upper]$. 

The combination of these scene variables forms a search space $\mathcal{D}$, which can be sampled to generate different scenes. However, these variables may have constraints that need to be included during sampling. For example, the structural variables such as road segments and waypoints may have sequential ordering constraints defined by the simulator's map. Similarly, temporal variables like the weather parameters (e.g., lighting) may have constraints on the rate at which their values change. In addition, each scene is associated with a risk score $S_{Risk}$ estimated by the risk estimator. Now, given the trained system with the calibrated risk estimator, we want to generate scenes in which the system is susceptible to failure. For this, our goal is to design a sampler that can address the following problems.    

% in the CARLA case study, the CARLA map defines the list of adjacent road segments, which forms the structural constraints. Similarly, there may be constraints on the rate of change in the values of the environmental variables. For example, the precipitation levels cannot drastically change from 10\% to 90\%, it can only gradually increase at a defined rate. Also, each scene is associated with a risk score $S_{Risk}$ estimated by the risk estimator. Given this set up, the goal is to test the \ac{cps} across scenes where it fails. For this, the goal of this work is to design a sampler that can address the following problems.  
    
\begin{problem}[Sample High-Risk Scene]
\label{prob:high-risk scene}
Given the scene variables $S_V$, the search space $\mathcal{D}$, and the sampling constraints, sample scenes $s_i$ that have risk $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from the previously observed scenes. 
\end{problem}

\begin{problem}[Sample Cluster of High-Risk Scenes]
\label{prob:cluster scene}
Given the scene variables $S_V$, the search space $\mathcal{D}$, and the sampling constraints, sample clusters of similar scenes $C_s$ that have risk $S_{Risk}$ $\geq$ $T_{Risk}$. Where $T_{Risk}$ is a threshold computed from the previously observed scenes 
\end{problem}

\textbf{Case Study}: We consider an \ac{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to explain these problems. In this example, an \ac{av} is tasked to navigate an urban town with complex traffic conditions, adverse weather conditions (e.g., high lighting level, high precipitation), and sensor faults (e.g., camera failure). These simulation parameters are the scene variables, which we sample to generate scenes with varying operating conditions. Also, to evaluate the \ac{av}'s performance, we leverage the infraction metrics returned by the CARLA autonomous driving challenge ~\cite{carla-challenge}. Specifically, we use the system infractions like running a red light, running a stop sign, route deviation, off-road driving, etc. Now, given this simulation setup, the goal of the \ac{av} is to navigate the different scenes without collisions. For this, the \ac{av} is augmented with several anomaly detectors, an \ac{ood} detector and a risk estimator~\cite{hartsell2021resonate} to estimate the \ac{av}'s risk of collision across an operating scene. The \ac{lec} controller is trained, and the risk estimator is calibrated using several train and calibration scenes. The specifics of the \ac{av} setup and training are discussed in \cref{sec:evaluation}. Now, given the trained \ac{av}, our goal is to find test scenes that are of high-risk to the \ac{av}. For this, our goal is to design a sampler that can address the two problems discussed above.




% Now, given the trained \ac{av}, we want to test it across different scenes where it is susceptible to failure. For this, our goal is to design a sampling approach that can sample. (1) scenes $s_i$ with different operating conditions and camera faults that has a risk greater than the risk across the training scenes. and (2) a cluster of scenes $C_s$ with similar operating conditions and camera faults that have a risk greater than the risk across the training scenes. 

% To address these problems, we design two sequential sampling approaches that considers the sampling constraints and provides an explicit control over the exploration and exploitation of the search space. The sampling approaches are discussed in the following section. 

% To explain these problems, we consider an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla}. We rely on the CARLA autonomous driving challenge ~\cite{carla-challenge} setup that allows simulating complex traffic scenes and it also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. This set up allows us to generate different traffic scenes by varying weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. In addition, it also allows us to inject different faults (e.g., camera occlusion, camera blur) into the \ac{av}'s sensors.  

% The \ac{av} in this set up is driven by a navigation \ac{lec} controller and it has an \ac{ood} detector and a \ac{resonate} risk estimator~\cite{hartsell2021resonate} as the safety components for runtime monitoring. The controller and the components are trained and calibrated using a set of scenes $\mathcal{T}$ generated by randomly varying the weather, traffic and pedestrian density, and road segments. Each of these scenes has an associated risk $R$ of \ac{av}'s collision as estimated by the risk estimator. Now, given simulator set up and the \ac{av}, the goal is to design a sampler that can find. (1) a single scene $s_i$ with different operating conditions and camera faults that has a risk greater than the risk across the training scenes, and (2) a cluster of scenes $C_s$ with similar operating conditions and camera faults that has a risk greater than the risk across the training scenes.     


% Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.

% \subsection{Case Study}
% We use an \acl{av} case study in CARLA simulator~\cite{dosovitskiy2017carla} to set up the problem. The \ac{av} is tasked to navigate an urban town with complex traffic scenarios including changing weather conditions, traffic density, and pedestrians density, which is designed for the CARLA autonomous driving challenge ~\cite{carla-challenge}. The \ac{av} uses a perception navigation \ac{lec} that uses the camera, \ac{imu}, \ac{gps}, and the speedometer sensors to predict the steer, throttle and brake control signals. In addition, it is augmented with several safety components like anomaly detectors, \ac{ood} detectors and risk estimator to access the system's risk during operation. Further, the setup also offers individual metrics to measure the infractions cause by the system like running a red light, running a stop sign, route deviation, off-road driving, etc. These metrics are combined to provide a single driving score to measure the \ac{av}'s driving proficiency.



==> individual-sections/rw.tex <==
\section{Related Work}
\label{sec:rw}
% The task of generating high-risk or safety critical scenes has been addressed in the literature using. 1) sampling-based approaches, 2) 

% can be broadly classified into three categories. 1) sampling

% The generation of high-risk or safety-critical scenes in simulation has gained significant interest in recent years. 
Tools like Dakota~\cite{dalbey2021dakota} with sampling approaches like incremental sampling, importance sampling, and adaptive sampling have been long available for uncertainty quantification in engineering design. Such samplers have recently gained interest for sampling simulation-based scenes in the \ac{av} domain. Several domain-specific \acp{sdl} like Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} have been designed for specifying scenarios of complex traffic conditions and operating conditions to identify edge cases and counterexamples that affect the system's safety. These languages are mostly designed for the \ac{av} domain to work with the CARLA simulator~\cite{dosovitskiy2017carla}. These languages are equipped with probabilistic samplers to sample values for scene variables from their distribution ranges, thus generating different scenes. For example, the Scenic language is integrated with the VERIFAI~\cite{dreossi2019verifai} software toolkit that has several passive samplers like random search, Halton search~\cite{halton1960efficiency}, and simulated annealing, which do not use the previous results to perform an informed sampling. Additionally, they include active samplers like cross-entropy optimization and \acl{bo}, which use a feedback loop of previous results in the sampling process. These samplers cannot control the exploration vs. exploitation tradeoff during sampling. To address this, a multi-armed bandit sampler that balances the two strategies is proposed~\cite{viswanadha2021parallel}. 

% As discussed by Ding, Wenhao, \emph{et al.}~\cite{ding2020learning}, g

There have also been other approaches. Grid search is a popular passive sampling approach used in industry. Here, a previously identified risky scene is used as the initial condition, and the grid around is searched to sample similar risky scenes. Manual tuning makes the grid sampler labor-intensive and time consuming. For accelerating the search process, an alternate approach~\cite{zhao2017accelerated} uses importance sampling to identify important scene variables and sample scenes using them. Worst-Case Scenario Evaluation~\cite{ma1999worst} is another approach that uses model-based optimization to identify the weakness of the system and uses this information to generate worst-case disturbances. 

In addition to the conventional samplers, there have recently been growing interests in using deep generative models for generating risky scenes~\cite{ding2018new,vardhan2021rare,o2018scalable,ding2020learning}. These approaches sample scenes from a learned distribution instead of sampling from the entire search space. Ding, Wenhao,\emph{et al.}~\cite{ding2020learning} use an autoregressive model to factorize the scene variables into conditional probability distributions, which are then sampled based on conditional dependence to generate risky traffic scenes. In a prior work~\cite{ding2018new}, they have also used a \acl{vae} to project high-dimensional traffic information into a lower-dimensional latent space, which is sampled to generate critical traffic scenes. Vardhan \emph{et al.}~\cite{vardhan2021rare} use a Gaussian Mixture Model to find the corner case scenes in the training set that is not well learned by the system. Another approach~\cite{o2018scalable} uses an ensemble of generative adversarial imitation learning to perform adaptive importance-sampling to learn rare events from an underlying data distribution. 



% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 















% The generation of scenes covering the entire range of expected environmental conditions has become an important study for testing and validating autonomous \ac{cps}. Scenic~\cite{fremont2019scenic} and MSDL~\cite{msdl} are well-known domain-specific \acp{sdl} used for scene generation. These languages have been equipped with probabilistic samplers to sample different values for the scene variables. Grid search is a brute force approach widely adopted in the industry. In this approach, a previously identified risky scene is used as the initial condition, and the grid around it is searched to sample risky scenes~\cite{ding2020learning}. This approach requires prior information of the risk scenes and can be labor-intensive. Instead of starting from manually identified risk scenes, an importance sampling approach for accelerated identification of high-risk scenes is proposed ~\cite{ding2020learning}. VERIFAI~\cite{dreossi2019verifai} provides several sampling approaches like random search, Halton search, cross-entropy optimization, and \acl{bo}, which is integrated with Scenic~\cite{fremont2019scenic} to generate scenes with counterexamples. Also, recently, the scene sampling process is formulated as a multi-armed bandit problem, which seeks to balance between exploration vs. exploitation ~\cite{viswanadha2021parallel,viswanadha2021addressing}.

% Recently, there has been growing interest in using generative models for sampling high-risk scenes. The central idea is to identify the high-risk distribution in the training set and then sample it to generate the high-risk scenes. The authors in~\cite{ding2020learning} have used \ac{gan} and \ac{vae} to identify high-risk distributions and sampling scenes from them. Similarly, Vardhan \emph{et al.}~\cite{vardhan2021rare} have used a Gaussian Mixture Model for learning the density of high-risk scenes from the training set. Then, samples are drawn from the learned model to generate high-risk scenes. However, most of these samplers do not employ a sequential search strategy. To include the past results in the selection process, the authors in~\cite{worstcaserl} have used Deep Q-learning based \acl{rl}. Here, the algorithm learns the policy of sampling scenes that maximize a reward function. 

==> results/comparison-table.tex <==
\begin{table}[!t]
\centering
\renewcommand{\arraystretch}{1.3}
\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Sampling\\ Approach\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Risk Scene \\ Percentage(\%)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Diversity\\ (No. of Clusters)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Search\\ Time (mins)\end{tabular}} \\ \hline
\textbf{Random}                                                      & 66                                                                            & 3                                                                              & 315                                                                   \\ \hline
\textbf{Halton}                                                      & 71                                                                            & 2                                                                              & 304                                                                   \\ \hline
\textbf{Grid}                                                         & 56                                                                            & 2                                                                             &306                                                                 \\ \hline
\textbf{RNS}                                                          & 83                                                                            & 6                                                                              & 335                                                                   \\ \hline
\textbf{GBO}                                                         & 92                                                                            & 4                                                                              & 897                                                                   \\ \hline
\end{tabular}
\caption{Comparison of the different sampling approaches in terms of the Risk Scene Percentage, Diversity and search time.}
\label{Table:comparison}
\vspace{-0.15in}
\end{table}

==> results/comparison-table1.tex <==
\begin{table}[!t]
\centering
\renewcommand{\arraystretch}{1.3}
\footnotesize
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Sampling\\ Appraoch\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Risk Scene \\ Percentage(\%)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{Diversity}}                                                                                          & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Search\\ Time (mins)\end{tabular}}} \\ \cline{3-4}
                                                                                      &                                                                                                & \begin{tabular}[c]{@{}c@{}}\textbf{\# of} \\ \textbf{Clusters}\end{tabular} & \textbf{\begin{tabular}[c]{@{}c@{}}Silhouette \\ score\end{tabular}} &                                                                                        \\ \hline
\textbf{Random}                                                                       & 66                                                                                             & 3                                                         & 0.34                                                                 & 433                                                                                    \\ \hline
\textbf{Halton}                                                                       & 71                                                                                             & 2                                                         & 0.27                                                                 & 395                                                                                    \\ \hline
\textbf{Grid}                                                                         & 56                                                                                             & 2                                                         & 0.71                                                                 & 405                                                                                    \\ \hline
\textbf{RNS}                                                                          & 83                                                                                             & 6                                                         & 0.56                                                                 & 900                                                                                    \\ \hline
\textbf{GBO}                                                                          & 92                                                                                             & 4                                                         & 0.62                                                                 & 906                                                                                    \\ \hline
\end{tabular}
\caption{Comparison of the different sampling approaches in terms of the Risk Scene Percentage, Diversity and search time.}
\label{Table:comparison}
\vspace{-0.15in}
\end{table}

==> results/faults.tex <==
\footnotesize
\begin{tabular}{c}
\hline
Sensor Faults                   \\ \hline%\hline
Center Cam Blur                   \\ %\hline
Left Cam Blur              \\ %\hline
Right Cam Blur  \\ %\hline
Center Cam Occlusion                 \\ %\hline
Left Cam Occlusion             \\ %\hline
Right Cam Occlusion 
              \\ \hline
\end{tabular}
% \caption{Simulation Variables and their distribution ranges.}
% \label{Table:variables}
% \vspace{-0.15in}


==> results/scene.tex <==
\footnotesize
\begin{tabular}{c|c}
\hline
Scene Variables             &  Range                    \\ \hline%\hline
Cloud                  & [0,100]                   \\ %\hline
Precipitation          & [0,100]              \\ %\hline
Precipitation deposits & [0,100]                         \\ %\hline
Time-of-day            & [0,90]                 \\ %\hline
Traffic density        & [0,20]             \\ %\hline
Pedestrian density     & [0,2]    \\
Road segments          & [0,9]                     \\ \hline
\end{tabular}
% \caption{Simulation Variables and their distribution ranges.}
% \label{Table:variables}
% \vspace{-0.15in}


==> symbols.tex <==
\begin{table}[!h]
    \centering
    % \setlength{\belowcaptionskip}{-6pt}
    \renewcommand{\arraystretch}{1.2}
    \footnotesize
    \begin{tabular}{|c|p{7.2cm}|}
    \hline
    Notation & Description\\
    \hline
    $s$ & scene \\
    \hline
    $s_v$ & scene variables \\
    \hline
    $v_d$ & variable distribution \\
    \hline
    $v_c$ & variable constraints \\
    \hline
    $\mathbb{E}$ & Environmental variables \\
    \hline
    $\mathbb{S}$ & Structural variables \\
    \hline
    $\mathbb{F}$ & Fault variables \\
    \hline
    $\mathcal{SC}$ & Sampling Constraints \\
    \hline
    $\lambda$ & dynamic hazard rate \\
    \hline
    $S_{Risk}$ & Risk Score \\
    \hline
    $RS$ & \ac{resonate} Score \\
    \hline
    $IS$ & Infraction Score \\
    \hline
    $\delta$ & Risk threshold computed across calibration set \\
    \hline
    $\mathcal{E}$ & List of previously explored scenes \\
    \hline
    $k$ & \ac{rns} sampler's parameter to control exploration vs. exploitation \\
    \hline
    $\beta$ & \ac{gbo} sampler's parameter to control exploration vs. exploitation \\
    \hline
    $P$ & Precipitation \\
    \hline
    $C$ & Cloudiness \\
    \hline
    $T$ & Time-of-day \\
    \hline
    $RS$ & Road Segments \\
    \hline
    $TD$ & Traffic Density \\
    \hline
    \end{tabular}
    \caption{Symbols used in the paper}
    \label{Table:SymbolTable}
    % \vspace{-0.4em}
\end{table}

